Markovian Interference in Experiments

We consider experiments in dynamical systems where interventions on some experimental units impact other units through a limiting constraint (such as a limited inventory). Despite outsize practical importance, the best estimators for this `Markovian' interference problem are largely heuristic in nature, and their bias is not well understood. We formalize the problem of inference in such experiments as one of policy evaluation. Off-policy estimators, while unbiased, apparently incur a large penalty in variance relative to state-of-the-art heuristics. We introduce an on-policy estimator: the Differences-In-Q's (DQ) estimator. We show that the DQ estimator can in general have exponentially smaller variance than off-policy evaluation. At the same time, its bias is second order in the impact of the intervention. This yields a striking bias-variance tradeoff so that the DQ estimator effectively dominates state-of-the-art alternatives. From a theoretical perspective, we introduce three separate novel techniques that are of independent interest in the theory of Reinforcement Learning (RL). Our empirical evaluation includes a set of experiments on a city-scale ride-hailing simulator.

==> Tex Files/Conclusion.tex <==
\section{Conclusion} \label{sec:real-conclusion}
We propose a novel estimator, the DQ estimator, to solve the interference problem in experiments with simple randomized designs. The DQ estimator achieves second-order bias in estimating the average treatment effect, while its variance can be exponentially smaller than that of any unbiased estimator. We conducted a large scale ride-hailing experiment that demonstrated the superior performance of the DQ estimator over state-of-the-art approaches. The striking and rigorous bias-variance trade-offs induced by the DQ estimator and its generalizations provide a new lens for general off-policy evaluation and policy optimization in reinforcement learning.


% Consider now the relationship  between Equation~\eqref{eq:dynkin-ate} (effectively, the idealized Off-Policy estimator) and the idealized Naive and DQ estimators:

% \begin{itemize}
%   \item Taking $\zeta(s) = 1$, we obtain the the idealized form of the DQ estimator: $\E_{\rho_{1 / 2}}\left[ Q_{\pi_{1 / 2}}(s, 1) - Q_{\pi_{1 / 2}}(s, 0)\right]$.
% \item Taking both $\zeta(s) = 1$ and $V_{\pi_{1 / 2}}(s) = c$ for any constant $c$, we obtain the idealized form of the Naive estimator $\E_{\rho_{1 / 2}}\left[ r(s, 1) - r(s, 0)\right]$.
% \end{itemize}

% These relationships immediately suggest that one  A variety of natural variance reduction techniques in fact provide levers for doing so:

% we can interpolate from DQ to Naive\footnote{The remaining possibility is to bias only the value function $V_{\pi_{1 / 2}}$ towards a constant, while using a consistent estimator for the likelihood ratio $\zeta$. The result would still be unbiased -- specifically, this yields the classical importance sampling estimator --- but this is known not to be efficient}.


% Note that this is an average-reward variant of the doubly-robust ``meta-estimator'' \cite{kallus2020double}, which captures as special cases various doubly-robust OPE estimators, and the closely-related primal-dual estimators.

% : biasing $\zeta(s)$ towards one interpolates between OPE and DQ, and further biasing $V_{\pi_{1 / 2}}$ towards any constant interpolates between DQ and Naive \footnote{The remaining possibility is to bias only the value function $V_{\pi_{1 / 2}}$ towards a constant, while using a consistent estimator for the likelihood ratio $\zeta$. The result would still be unbiased -- specifically, this yields the classical importance sampling estimator --- but this is known not to be efficient}. A variety of common variance reduction techniques fit in this framework, yielding one of OPE, DQ or Naive as extremes.

%  {\it Function approximation}. Consider {\em approximate} estimation of the value function via state aggregation, for example in cases where the state space is massive. A typical strategy here is function approximation; that is, to constrain the estimated value function $\hat{V}$ to lie in a particular function class. Intuitively, simpler function classes admit higher bias but lower variance estimates of the ATE. One extreme is to allow $\hat{V}$ to be an arbitrary function of state, which allows us to recover the ideal DQ estimator in the limit; at the other extreme, if we constrain $\hat{V}$ to be a constant (alternatively, this can be interpreted as aggregating all states into a single aggregate state; or regularizing $\hat{V}$ towards a constant value), we then recover exactly the naive estimator:

% \begin{proposition}
%   Let $\hat{V} = {\bf 1} c$ for any constant $c$. Then, $\hat{\mathrm{ATE}}_{D} = \hat{\mathrm{ATE}}_{N}$.
% \end{proposition}

% Controlling the complexity of the value function approximation interpolates between the DQ and Naive estimators.

% {\it Discounting.} A common technique to estimate the average reward value function is to instead estimate a  discounted reward value function $Q_{\gamma}(s, a) = \mathbb{E}\left[\sum_{t=0}^T \gamma^{t} r(s_t, a_t) | s_{0} = s, a_0 = a\right]$, motivated by the fact that, under the proper scaling, we obtain exactly the average-reward value function $Q$ as the discount rate $\gamma$ goes to one (precisely,  $\lim_{\gamma \to 1} (1 - \gamma) Q_{\gamma}(s, a) = Q(s, a)$ \cite{putermanMarkovDecisionProcesses2014}). This approach is commonly applied to reduce variance (see e.g. \cite{kakade2001optimizing}).

% Consider now implementing the DQ estimator, using the biased discounted estimator $(1-\gamma)V_{\gamma}(s)$. At one extreme, as we take $\gamma \to 1$, we recover the exact DQ estimator; at the other extreme of $\gamma = 0$,  $Q_{\gamma}(s, a) = r(s, a)$ and we recover the Naive estimator.

% \textbf{Regularization and the OPE meta-estimator:} We now look to the other side of the bias va

% As Theorem~\ref{th:dynkin_var}, and Theorem~\ref{th:cramer-rao} show, the difference in variance between estimating Equation~\eqref{eq:dynkin-ate} with and without the likelihood ratios (i.e., between DQ and unbiased OPE) can be massive. This immediately suggests a method of interpolating along the bias-variance curve between these two estimators: simply regularize estimates of the likelihood ratio towards one. Recent regularized primal-dual OPE algorithms (e.g.~\cite{nachum2019dualdice}) have in fact realized empirical performance gains from such regularization.

% Revisiting the off-policy meta-estimator and its prohibitively large variance resulting from estimating likelihood ratios, one practical approach to wrangling that variance is {\em regularization} -- loosely speaking, a greater level of regularization should lower the variance while introducing bias. One nice observation here is that the DQ estimator can be thought of as the extreme case of this strategy, where the likelihood ratios are regularized to being identically one. This lens in principle allows us to attain the entire bias-variance `curve' from the OPE meta-estimator to the DQ estimator.

% Relative to this meta-estimation strategy based on Dynkin's formula, our theory that the DQ estimator pays a low cost in bias (Theorem~\ref{th:dynkin_bias}) for a potentially exponential improvement in variance (Theorem~\ref{th:dynkin_var}, and Theorem~\ref{th:cramer-rao} in the next section.).

% Doubly

% This identity is (a special case of) {\em Dynkin's formula} {\cite{dynkin1965markov}, and is a critical step in showing our bias bound (Theorem \ref{th:dynkin_bias}).

%   Connecting to the policy optimization literature, Dynkin's formula is a frequently used tool (e.g.~\cite{kakade2002approximately,schulman2015trust}), even if not always named explicitly.

%   For more intuition, consider that the above identity immediately implies the following identity on the ATE:
%  A large family of off-policy estimators estimate \eqref{eq:dynkin-ate} by plugging-in estimators for both the likelihood ratio and $Q_{\pi_{1 / 2}}$, % model complexity in $Q$-function estimation immediately translates to an
 % interpolation between the DQ and Naive estimators.

% As in the previous point, the bias-variance curve between the DQ and Naive estimators is also in principle attainable. To see this, consider {\em approximate} estimation of the $Q$-function -- this is necessary when the state space is massive, as was the case in our ridesharing experiments. The extent to which one can trade off between estimation accuracy and   %Thus, as in the previous point bias-variance `curve' between the DQ and Naive estimators is in principle attainable.

% To conclude, we touch on two practical considerations when implementing the DQ estimator. These also directly connect the DQ estimator to the unbiased (but high-variance) off-policy meta-estimator described in Section \ref{sec:connection}, and the low-variance (but high-bias) Naive estimator.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> Tex Files/Estimator.tex <==
%\documentclass[]{article}
%\usepackage[]{amsmath,amssymb}
%\begin{document}
\section{The Differences-In-Q's Estimator}
\label{sec:estimator}

We are now prepared to introduce our estimator for inference in the presence of Markovian interference.
%Our choice of name rests on the fact that calculating the bias of this estimator (which we show to be small) relies on Dynkin's formula, an identity that has been rediscovered many times in the RL literature. 
Before defining our estimator, which we will see is only slightly more complicated than the Naive estimator, we recall a few useful objectis in average-reward MDPs. Denote the average cost of a policy $\pi$ by $\lambda^{\pi}$. The $V$-function of a policy $\pi$, $V_{\pi}$, characterizes the ``reward-to-go'' $V_{\pi}(s) := \E\Big[\sum_{t=0}^{\infty} r(s_t, a_t) - \lambda^{\pi}~\big|~s_0 = s\Big].$
% Do we need to define this anywhere?
It is also known that $(V_{\pi}, \lambda^{\pi})$ is the fixed point of the Bellman operator $T_{\pi}$ with $T_{\pi}(V_{\pi}, \lambda^{\pi}) = V_{\pi}.$ Here $T_{\pi}: \mathbb{R}^{|\Sscr|} \times \mathbb{R} \rightarrow \mathbb{R}^{|\Sscr|}$ is given by $T_\pi (V, \lambda)  = r_\pi - \lambda \mathbf{1} + P_{\pi} V$ where $r_\pi: \Sscr \rightarrow \mathbb{R}$ is defined according to $r_\pi(s) = \E\left[r(s, \pi(s))\right]$.
%The average cost of policy $\pi$, denoted $\lambda^\pi$, and the bias function corresponding to $\pi$, denoted $V_{\pi}$, are then a solution to the fixed point equation $T_\pi (V, \lambda)  = V$. 
Finally, the $Q$-function associated with $\pi$, denoted $Q_\pi: \Sscr \times \Ascr \rightarrow \mathbb{R}$, is defined according to $Q_\pi(s,a) := \E\Big[\sum_{t=0}^{\infty} r(s_t, a_t) - \lambda^{\pi}~\big|~s_0 = s, a_0 = a\Big]$. Put simply, the $Q$-function measures the `excess' reward obtained starting from $s$ with the action $a$ relative to the average reward under $\pi$. 

\subsection{An Idealized First Step}
In motivating our estimator, let us begin with the following idealization of the Naive estimator, where we denote by $\rho_{1/2}$ the steady state distribution under the randomization policy $\pi_{1/2}$: $\E_{\rho_{1/2}} \left[\hat {\rm ATE}_{\rm NV}\right] = \sum_s \rho_{1/2}(s) \left[ r(s,1) - r(s,0)\right].$ It is not hard to see that in the example of Section~\ref{sec:example}, we continue to have $\lvert \E_{\rho_{1/2}} [\hat {\rm ATE}_{\rm NV} ] - {\rm ATE} \rvert \approx \frac{p\lambda}{\mu} \mathrm{ATE}$, i.e. this idealization of the Naive estimator continues to have bias on the order of the treatment effect. Consider then, the following alternative:
\[
\E_{\rho_{1/2}} \left[\tauDK\right] = \sum_s \rho_{1/2}(s) \left[Q_{\pi_{1/2}}(s,1) - Q_{\pi_{1/2}}(s,0)\right],
\]
where the term $\E_{\rho_{1/2}} [\tauDK]$ can for now just be thought of as an idealized constant ($\tauDK$ is defined soon in \eqref{eq:Dynkin}).
Compared to $\E_{\rho_{1/2}} [\hat {\rm ATE}_{\rm NV}]$, we see that $\E_{\rho_{1/2}} [\hat {\rm ATE}_{\rm DQ}]$  takes a remarkably similar form, except that as opposed to an average over differences in rewards, we compute an average of differences in $Q$-function values. The idea is that doing so will hopefully compensate for the shift in distribution induced by $\pi_{1/2}$, as it does in the example of Section~\ref{sec:example}.
%{\em Crucially, we rely on the $Q$-function  corresponding to $\pi_{1/2}$}. Since the experiment generates data under this very policy, it tuns out that these $Q$-values are substantially easier to estimate. 
% \begin{example}[Continued]
% Continuing with our example, we can explicitly calculate $Q_{\pi_{1/2}}(\cdot,\cdot)$, the average reward $\lambda^{\pi_{1/2}}$, and the stationary distribution $\rho_{1/2}$  (see Appendix \ref{sec:calculation-example}). Doing so allows us to calculate that
% \[
% \E_{\rho_{1/2}} \left[
% \hat {\rm ATE}_D
% \right]
% =
% \frac{1}{2} \left(
% \frac{\delta}
% {(1 - \delta/2)^2}
% \right).
% \]
% That is, $|{\rm ATE} - \E_{\rho_{1/2}} [\hat {\rm ATE}_D]| = O(\delta^2)$,
% so that the bias of this idealized estimator is second-order (i.e. negligible) relative to the {\em ATE}.
% \end{example}

Is the dramatic mitigation of bias we see in the example generic? If the experimentation policy mixes fast, our first set of results essentially answers this question in the affirmative. In particular, we make the following mixing time assumption:

%\begin{assumption}
%[Transitions]
%We assume that the change in distribution over next states under the intervention is Lipschitz in the treatment effect. Specifically, for any state $s \in \Sscr$,  
%\[
%d_{\rm TV}( p(s,1,\cdot), p(s,0,\cdot) ) \leq L \delta 
%\]
%where $L$ is a Lipschitz constant and $\delta$ is the $ATE$.   
%\end{assumption} 
%The above assumption is relatively benign. In particular, the condition is trivially satisfied for the examples in $\cite{}$. Our first result concerns the bias of the Dynkin estimator, which we show is small: 

\begin{assumption}[Mixing time]\label{assump:mixing-time}
There exist constants $C$ and $\lambda$ such that for all $s \in \Sscr$, $d_{\rm TV} (P_{1/2}^{k}(s, \cdot), \rho_{1/2}) \leq C \lambda^{k}$ where $d_{\rm TV}(\cdot,\cdot)$ denotes total variation distance.
\end{assumption}

We then have that the second order bias we saw in Section~\ref{sec:example} is, in fact, generic:

\begin{theorem}[Bias of DQ]
\label{th:dynkin_bias}
Assume that for any state $s \in \Sscr$,  
$
d_{\rm TV}( p(s,1,\cdot), p(s,0,\cdot) ) \leq \delta. 
$
Then,
\[
\left|{\rm ATE} - \E_{\rho_{1/2}} \left[
\hat {\rm ATE}_{\rm DQ}
\right]\right| \leq C' \left(\frac{1}{1-\lambda}\right)^2 r_{\max} \cdot \delta^2
\]
where $r_{\max} := \max_{s,a} \left|r(s,a)\right|$ and $C'$ is a constant depending (polynomially) on $\log(C)$.
\end{theorem}
%\subsubsection{Proof outline of Theorem \ref{th:dynkin_bias}}
% The proof of \cref{th:dynkin_bias} relies on the following Taylor expansion of the average reward around $P_{1/2}$:
% \begin{lemma}[Taylor expansion of the average reward.]
%   \label{lem:taylor}
%   For any $K \in \mathbb{N}$, it holds that
%   \begin{equation*}
%     \lambda^{\pi_{1}} = \sum_{k=0}^{K} \delta^{k} \rho_{1 / 2}^{\top} \left( \Delta (I - P_{\pi_{1 / 2}})^{\#} \right)^{k} r_{1} + o(\delta^{K})
%   \end{equation*}
%   where $r_{1}$ is the vector $\{r(s, 1)\}_{s \in \mathcal{S}}$, and $\delta\Delta = P_{\pi_{1}} - P_{\pi_{1 / 2}} $.
% \end{lemma}
% This Lemma immediately motivates both the Naive estimator



\subsection{The Differences-In-Q's Estimator}

Motivated by the development in the previous subsection, the {\em Differences-In-Q's (DQ)} estimator we propose to use is simply 
\begin{equation}
\label{eq:Dynkin}
\hat {\rm ATE}_{\rm DQ}
= 
\frac{1}{|T_1|}
\sum_{t \in T_1}
\hat Q_{\pi_{1/2}}(s_t,a_t)
-
\frac{1}{|T_0|}
\sum_{t \in T_0}
\hat Q_{\pi_{1/2}}(s_t,a_t),
\end{equation}
where we take an empirical average over the state trajectory produced under the randomization policy, and $\hat Q_{\pi_{1/2}}$ is an estimator of the $Q$-function. For concreteness, we obtain $\hat Q_{\pi_{1/2}}$ by solving
\begin{align}\label{eq:LSTD0-V}
\min_{\hat V, \hat \lambda}
\sum_{s \in \Sscr} 
\left(\sum_{t, s_{t}=s} 
r(s_t, a_t) - \hat{\lambda} + \hat V(s_{t+1}) - \hat V(s_t)
\right)^2.
\end{align}
Our main result characterizes the variance and asymptotic normality of $\hat {\rm ATE}_{\rm DQ}$:
\begin{theorem}[Variance and Asymptotic Normality of DQ]
\label{th:dynkin_var}
The DQ estimator is asymptotically normal so that $
\sqrt{T}
\left(\hat {\rm ATE}_{\rm DQ} - \E_{\rho_{1/2}} \left[\hat {\rm ATE}_{\rm DQ}\right]\right) \overset{d}{\rightarrow} \mathcal{N}(0, \sigma_{\rm DQ}^2),
$
with limiting standard deviation 
\[
\sigma_{\rm DQ} \leq C'\left(\frac{1}{1-\lambda}\right)^{5/2} \log \left( \frac{1}{\rho_{\min}}\right) r_{\max}.
\]
where $\rho_{\min} := \min_{s\in S} \rho_{1/2}(s)$ and $C'$ is a constant depending (polynomially) on $\log(C)$. 
\end{theorem}

The fact that $\sigma_{\rm DQ}$ in \cref{th:dynkin_var} only depends on $1/\rho_{\min}$ logarithmically is somewhat surprising. In fact, a coarse analysis will lead to $\sigma_{D} = \Omega\left(\frac{1}{\rho_{\min}}\right)$, which shows no advantage compared to the unbiased OPE estimators (which we will see momentarily). The key enabler for this striking result is a novel lemma that exploits an \textit{entry-wise bound} for controlling the variance, even at states that are rarely visited (we dub this the ``Entry-wise Non-expansive Lemma''; see \cref{lem:non-expansive-lemma}). The lemma admits a simple form and may have broader implications for analyzing variance in OPE estimators (see Discussions in \cref{sec:conclusion}). In addition, our asymptotic normality analysis borrows the delta-method framework used in the context of on-policy LSTD \cite{konda2002actor}, but with a novel linearization that dramatically simplifies the analysis. See \cref{sec:proof-sketch-dynkin-var} for more details. 

\noindent\textbf{\textsf{One Extreme of the Bias-Variance Tradeoff:}} We may heuristically think of the Naive estimator as representing one extreme of the bias-variance tradeoff among reasonable estimators. For the sake of comparison, by the Markov Chain CLT, the Naive estimator is also asymptotically normal with standard deviation $\Theta (r_{\rm max}/ (1-\lambda)^{1/2})$. This rate is efficient for the estimation of the mean of a Markov chain \cite{greenwood1995efficiency}. On the other hand, while the Naive estimator is effectively useless for the problem at hand given its bias is in general $\Theta(\delta)$, that of the DQ estimator is $O(\delta^2)$.

\subsection{Proof of \cref{th:dynkin_bias}}\label{sec:proof-of-dynkin-bias}
The proof of \cref{th:dynkin_bias} is a simple proof built on a perturbation formula for stationary distributions of Markov chains. We in fact construct a novel Taylor series representation of the ATE parameterized by $\delta$ that controls the perturbation around $P_{1 / 2}$, which yields the Naive estimator as the zeroth-order truncation of the series; and the idealized DQ estimator as the natural first-order correction. \cref{th:dynkin_bias} then proceeds by bounding the remainder. This strategy additionally allows us to generalize the DQ estimator to arbitrarily high-order bias corrections, by computing $Q$-functions iteratively. Here we present the proof (with some details omitted for simplicity). %These results can be of independent interest for the field of OPE and policy optimization. See proof details in \cref{sec:proof-of-dynkin-bias}.
%The proof is a simple proof based on observing a particular way of parameterizing ATE as a function of $\delta$. Turns out the Taylor expansion of such a function reveals naturally the bias-correction results of corresponding estimators (Naive estimator is the zeroth-order Taylor truncation, the DQ estimator is the first-order Taylor truncation, et.al). 

We first define few pieces of useful notation. Let $\rho_{0} \in \R^{|\Sscr|}, \rho_{1/2} \in \R^{|\Sscr|}, \rho_{1} \in \R^{|\Sscr|}$ be the vectors of the stationary distributions of $P_0, P_{1/2}, P_{1}$ accordingly. Let $r_0 \in \R^{|\Sscr|}, r_{1/2} \in \R^{|\Sscr|}, r_1 \in \R^{|\Sscr|}$ be the reward vectors associated with policies $\pi_0, \pi_{1/2}, \pi_{1}$, i.e., $r_{a}(s) = r(s, a)$ and $r_{1/2} = \frac{1}{2} r_0 + \frac{1}{2} r_1.$

To begin, we parameterize $P_0 := P_{1/2} - \delta A$ and $P_1 := P_{1/2} + \delta A$ by $\delta$ with fixed $P_{1/2}$ and some fixed matrix $A \in \R^{|\Sscr|\times |\Sscr|}$ with $\|A\|_{1,\infty} \leq 1$ ($\|A\|_{1,\infty} = \max_{i}\sum_{j}|A_{ij}|$)\footnote{This is always possible since $d_{\rm TV}( p(s,1,\cdot), p(s,0,\cdot) ) \leq \delta.$ }. Then, $\rho_{0}$ and $\rho_{1}$ can also be viewed as a function of $\delta.$ Also recall ${\rm{ATE}} = \rho_{1}^{\top} r_{1} - \rho_{0}^{\top} r_0$. Our goal is to represent ${\rm{ATE}}$ as a function of $\delta$ and then study the Taylor expansion of such a function. To do so, we use the following known perturbation formula of Markov chains.
\begin{lemma}[Stationary Distribution Perturbation, Theorem 4.1 \cite{meyer1980condition}]\label{lem:perturbation-stationary-distribution}
Suppose $P \in \R^{n \times n}$ and $P' \in \R^{n\times n}$ are transitions matrices of two finite-state aperiodic and irreducible Markov Chains and $\rho \in \R^{n}, \rho' \in \R^{n}$ are the stationary distributions accordingly. Then $\rho'^{\top} = \rho^{\top} + \rho'^{\top} (P' - P) (I - P)^{\#}$ 
where $(I-P)^{\#}$ is the group inverse of $I-P$ given by $(I-P)^{\#}=(I-P+\one \rho^{\top})^{-1} - \one \rho^{\top}.$
\end{lemma}
Let us apply \cref{lem:perturbation-stationary-distribution} to $\rho_{1}^{\top} r_1$ based on the perturbation between $\rho_{1/2}$ and $\rho_{1}$.
\begin{align}
\rho_1^{\top} r_1 
&= \rho_{1/2}^{\top} r_1 + \rho_{1}^{\top} (P_1 - P_{1/2}) (I-P_{1/2})^{\#} r_1 \nonumber\\
&= \rho_{1/2}^{\top} r_1 + \delta \cdot \rho_{1}^{\top} A (I-P_{1/2})^{\#} r_1 \label{eq:expansion-rho-rho1}
\end{align}
Note that we can apply \cref{lem:perturbation-stationary-distribution} again to the $\rho_{1}$ in the RHS of \cref{eq:expansion-rho-rho1} and then repeat this process, 
\begin{align}
\rho_1^{\top} r_1 
&= \sum_{k=0}^{K} \delta^{k} \cdot \rho_{1/2}^{\top} \left(A (I-P_{1/2})^{\#}\right)^k r_1 + \delta^{K+1} \cdot \rho_{1}^{\top} \left(A (I-P_{1/2})^{\#}\right)^{K+1} r_1 \label{eq:expansion-rho-rho1-K}
\end{align}
for any $K = 0, 1, 2, \dotsc$. Essentially \cref{eq:expansion-rho-rho1-K} provides the $K$-th order Taylor expansion for $\rho_{1}^{\top}r_1$ with an explicit remainder. Furthermore, we can bound the remainder by
\begin{align*}
\left|\rho_{1}^{\top} \left(A (I-P_{1/2})^{\#}\right)^{K+1} r_1\right| 
&\overset{(i)}{\leq} \norm{\rho_{1}}_{1} \left(\norm{A}_{1,\infty} \norm{I-P_{1/2}^{\#}}_{1,\infty}\right)^{K+1} \norm{r_1}_{\max}\\
&\overset{(ii)}{\leq} \norm{I-P_{1/2}^{\#}}_{1,\infty}^{K+1} r_{\max} \\
&\overset{(iii)}{\leq} \left(\frac{2\ln(C)+1}{1-\lambda}\right)^{K+1} r_{\max}
\end{align*}
Here in (i) we use that for any vector $a, b$ and matrix $B$, we have $|a^{\top}b| \leq \|a\|_{1}\|b\|_{\max}$ and $\norm{a^{\top}B}_{1} \leq \norm{a}_{1} \norm{B}_{1,\infty}$. In (ii) we use that $\norm{\rho_1}_1 = 1, \norm{A}_{1,\infty} \leq 1$. In (iii), we use the following lemma implied by the mixing time assumption and the series expansion of $(I-P)^{\#}.$
\begin{lemma}\label{lem:group-inverse-L1}
    Suppose for any $s \in \Sscr$, $d_{\rm TV} (P^{k}_{1/2}(s, \cdot), \rho_{1/2}) \leq C \lambda^{k}$. Then $\norm{(I-P_{1/2})^{\#}}_{1,\infty} \leq \frac{2\ln(C)+1}{1-\lambda}.$
\end{lemma}

Appplying a similar process to $\rho_{0}^{\top}r_0$, we obtain the Taylor expansion for the ATE.
\begin{align}
{\rm{ATE}} 
%&= \rho_1^{\top} r_1 - \rho_0^{\top} r_0 \nonumber\\
&=  \sum_{k=0}^{K} \delta^{k} \cdot \left(\rho_{1/2}^{\top} \left(A (I-P_{1/2})^{\#}\right)^k r_1 - \rho_{1/2}^{\top} \left((-A) (I-P_{1/2})^{\#}\right)^k r_0\right) + \delta^{K+1} \cdot a_{K} \label{eq:taylor-expansion-ATE}
\end{align}
where $|a_{K}| \leq 2\left(\frac{2\ln(C)+1}{1-\lambda}\right)^{K+1} r_{\max}.$ It is easy to see that the Naive estimator $\rho_{1/2}^{\top}(r_1-r_0)$ corresponds to the zeroth-order truncation. In fact, the DQ estimator, i.e., $\E_{\rho_{1/2}} \left[\tauDK \right]$, exactly matches the first-order truncation. To see this, by the definition of $\E_{\rho_{1/2}} \left[\tauDK \right]$ and $Q$-functions, 
\begin{align*}
\E_{\rho_{1/2}} \left[\tauDK \right] 
&= \sum_s \rho_{1/2}(s) \left(Q_{\pi_{1/2}}(s,1) - Q_{\pi_{1/2}}(s,0) \right) \\
&= \sum_{s} \rho_{1/2}(s) \left(r_1(s) +\sum_{s'} V_{1/2}(s')P_{1}(s,s') - r_0(s) - \sum_{s'} V_{1/2}(s')P_{0}(s,s')\right)\\
&= \rho_{1/2}^{\top} \left(r_1 - r_0 + (P_1-P_0)V_{1/2}\right)
\end{align*}
where $V_{1/2}$ is the induced vector of the $V$-function of policy $\pi_{1/2}.$ By the well-known fact that $V_{1/2} = (I-P_{1/2})^{\#} r_{1/2}$ induced by the Bellman equation, we then have
\begin{align*}
\E_{\rho_{1/2}} \left[\tauDK \right] 
&=  \rho_{1/2}^{\top} \left(r_1 - r_0 + (P_1-P_0)(I-P_{1/2})^{\#} r_{1/2}\right)\\
&= \rho_{1/2}^{\top} r_1  - \rho_{1/2}^{\top} r_0 + \delta \rho_{1/2}^{\top}A (I-P_{1/2})^{\#} (r_{1}+r_{0}).
\end{align*}
Then indeed $\E_{\rho_{1/2}} \left[\tauDK \right]$ is the first-order Taylor truncation. Together, this completes the proof.
%\begin{align*}
%\left|{\rm{ATE}} - \E_{\rho_{1/2}} \left[\tauDK \right]\right| \leq 2\delta^2 r_{\max}\left(\frac{2\ln(C)+1}{1-\lambda}\right)^2.
%\end{align*}
\noindent\textbf{\textsf{Generalization to Higher-Order Bias Correction.}} In fact, the K-th order Taylor expansion of ATE allows us to design estimators that can correct higher-order bias, based on computing difference-in-Q functions iteratively. See details in \cref{sec:korder-correction}.

\subsection{Proof Sketch of \cref{th:dynkin_var}}\label{sec:proof-sketch-dynkin-var}
We aim to use the Markov chain CLT (\cite{jones2004markov}) to show asymptotic normality of our estimator. The Markov chain CLT states that for a Markov chain $X_{1}, X_{2}, \dotsc, $ and a bounded function $u$ with domain on the state space, there exists $\Sigma_{u}$ such that $\sqrt{T}\left(\frac{1}{T}\sum_{t=1}^{T} u(X_t) - u^{*}\right) \overset{d}{\rightarrow} N(0, \Sigma_{u})$
where $u^{*}$ is the expected value of $u$ under the stationary distribution of the Markov chain. See proof details in \cref{sec:proof-variance-bound}.

\noindent\textbf{\textsf{Delta method.}} Unfortunately, the estimator $\tauDK$ can not be directly written as an empirical average of some function $u.$ To address this issue, we use the the delta method (traced back to \cite{doob1935limiting}, see \cref{lem:mapping-CLT}). In particular, we write $\tauDK = f(u_T)$ as a function of a random vector $u_{T}$ given by $u_{T} := \frac{1}{T}\sum_{t=1}^{T} u(X_{t}).$ Under some minor conditions, the delta method states that $\sqrt{T} \left(f(u_{T}) - f(u^{*})\right) \overset{d}{\rightarrow} N(0, \sigma_{f}^2)$
where $\sigma_{f}^2 := \nabla f(u^{*})^{\top} \Sigma_{u} \nabla f(u^{*})$ and $\nabla f(u^{*})$ is the gradient of $f$ evaluating at the point $u^{*}.$ This forms the basis for proving \cref{th:dynkin_var}.

\noindent\textbf{\textsf{Linearization.}} To simplify the analysis for $\sigma_{f}$, instead of computing $\Sigma_{u}$ explicitly, we ``linearize'' the function $f$ by defining $\tilde{f}(X_{t}) := \nabla f(u^{*})^{\top}(u(X_t)-u^{*})$ and the delta method in fact implies (see \cref{lem:linearization}) $\sqrt{T}\left(\frac{1}{T}\sum_{t=1}^{T} \tilde{f}(X_t)\right) \overset{d}{\rightarrow} N(0, \sigma_{f}^2),$
i.e., the linearized $f$ converges with the same limiting variance as the original $f.$ Therefore, we can focus on $\tilde{f}$ for analyzing $\sigma_{f}.$ 

\noindent\textbf{\textsf{Bounding $\sigma_f$ with Entry-wise Non-expansive Lemma.}} To bound $\sigma_{f}$, we will invoke \cref{lem:bound-for-sigma}, which states that $\sigma_{f} \leq \sqrt{2}\sqrt{\frac{2\ln(C)+1}{1-\lambda}}\tilde{f}_{\max}$
where $\tilde{f}_{\max} := \max_{s} |\tilde{f}(s)|.$ Then the problem reduces to bounding $\tilde{f}_{\max}$, which will be controlled by the following key lemma.
\begin{lemma}[Entry-wise non-expansive lemma]\label{lem:non-expansive-lemma}
Let $W: \R^{|\Sscr|} \rightarrow \R^{|\Sscr|}$ be a map denoted by $W(\rho) := (I-P_{1/2})^{\#\top}(P_1-P_0)^{\top} \rho.$ Let $c := 4\frac{\ln(C) +  \ln \left(1/\rho_{\min}\right) + 1}{1-\lambda}.$ Then, for any $s \in \Sscr$,  $\frac{1}{c}\left|W(\rho_{1/2}) (s)\right| \leq \rho_{1/2}(s).$
\end{lemma}


%In contrast, we see that the standard deviation of the DQ estimator is only larger by a logarithmic factor. 
%\textbf{Proof Technique:} The asymptotic normality is established 

% \subsection{Connections to an off-policy meta-estimator via Dynkin's formula} \label{sec:connection}

% Having formally defined our estimator, we can now expand on some of the connections to the RL literature described earlier, particularly to policy optimization and off-policy estimation. One identity that is critical to making both connections apparent is the following:
% \begin{equation*}
%  \lambda^{\pi_1}  = \lambda^{\pi_{1/2}} + \frac{1}{2}\E_{\rho_{1 / 2}}\left[\frac{\rho_{1}(s)}{\rho_{1 / 2}(s)} \left(Q_{\pi_{1 / 2}}(s, 1) - Q_{\pi_{1 / 2}}(s, 0) \right)\right],
% \end{equation*}
% with the same identity holding if $\pi_1$ and $\rho_1$ are replaced with $\pi_0$ and $\rho_0$. This identity is (a special case of) {\em Dynkin's formula} {\cite{dynkin1965markov}, and is a critical step in showing our bias bound (Theorem \ref{th:dynkin_bias}). Connecting to the policy optimization literature, Dynkin's formula is a frequently used tool (e.g.~\cite{kakade2002approximately,schulman2015trust}), even if not always named explicitly. For more intuition, consider that the above identity immediately implies the following identity on the ATE:
% \begin{equation}
%   \label{eq:dynkin-ate}
%  \mathrm{ATE} = \E_{\rho_{1 / 2}}\left[\frac{(1 / 2) (\rho_{1}(s) + \rho_{0}(s))}{\rho_{1 / 2}(s)} (Q_{\pi_{1 / 2}}(s, 1) - Q_{\pi_{1 / 2}}(s, 0))\right].
% \end{equation}
% This is a familiar expression: it is precisely the DQ estimator, but with a likelihood ratio correction at each state to yield an unbiased estimator. A large family of off-policy estimators estimate \eqref{eq:dynkin-ate} by plugging-in estimators for both the likelihood ratio and $Q_{\pi_{1 / 2}}$, including doubly robust estimators (see e.g.~\cite{kallus2020double,ueharaMinimaxWeightQFunction2020}), as well as the closely-related primal-dual estimators (see \cite{daiBoostingActorDual2017,tangDoublyRobustBias2019} for connections to the doubly robust literature). Relative to this meta-estimation strategy based on Dynkin's formula, our theory that the DQ estimator pays a low cost in bias (Theorem~\ref{th:dynkin_bias}) for a potentially exponential improvement in variance (Theorem~\ref{th:dynkin_var}, and Theorem~\ref{th:cramer-rao} in the next section.).
%
%
%A large family of OPE estimators have tight connections to Dynkin's formula, including doubly robust estimators (see e.g.~\cite{kallus2020double,ueharaMinimaxWeightQFunction2020}), as well as the closely-related primal-dual estimators (see \cite{daiBoostingActorDual2017,tangDoublyRobustBias2019} for connections to the doubly robust literature). Translated to the average-reward setting, the population estimating equation for these estimators is:
%
%\begin{equation*}
% \lambda_{1}  = \lambda_{1 / 2} + \E_{\rho_{1 / 2}}\left[\frac{\rho_{1}(s)}{\rho_{1 / 2}(s)} \left(Q_{\pi_{1 / 2}}(s, 1) - V_{\pi_{1 / 2}}(s) \right)\right]
%\end{equation*}
%
%where in practice the expectation and the nuisance parameters $\rho_{1}, \rho_{1 / 2}, \lambda_{1 / 2}, Q_{\pi_{1 / 2}}, V_{\pi_{1 / 2}}$ must be estimated. % either using plug-in regression estimators, or by solving a saddle point problem.
%
%More specifically, under our experimentation policy we have $V_{\pi_{1 / 2}}(s) = \frac{1}{2} Q_{\pi_{1 / 2}}(s, 1) + \frac{1}{2} Q_{\pi_{1 /2}}(s, 0)$ and the expression above reduces to
%\begin{equation*}
% \lambda_{1}  = \lambda_{1 / 2} + \frac{1}{2}\E_{\rho_{1 / 2}}\left[\frac{\rho_{1}(s)}{\rho_{1 / 2}(s)} \left(Q_{\pi_{1 / 2}}(s, 1) - Q_{\pi_{1 / 2}}(s, 0) \right)\right]
%\end{equation*}
%
%Finally, computing the estimate $\lambda_{1} - \lambda_{0}$ yields a familiar expression:
%
%\begin{equation*}
% \lambda_{1} - \lambda_{0} = \E_{\rho_{1 / 2}}\left[\frac{(1 / 2) (\rho_{1}(s) + \rho_{0}(s))}{\rho_{1 / 2}(s)} (Q_{\pi_{1 / 2}}(s, 1) - Q_{\pi_{1 / 2}}(s, 0))\right]
%\end{equation*}
%
%This is precisely the Dynkin estimator, but with a likelihood ratio correction at each state to yield an unbiased estimator. Relative to the DR estimator, our theory demonstrates that the Dynkin estimator pays a low cost in bias (Theorem~\ref{}) for a potentially exponential improvement in variance.
%
%


%\subsection{The estimator and bias}
%
%The Dynkin estimator is simply:
%\begin{equation}
%\label{eq:Dynkin}
%\hat {\rm ATE}_D
%= 
%\frac{1}{|T_1|}
%\sum_{t \in T_1}
%Q_{\pi_p}(s_t,a_t)
%-
%\frac{1}{|T_0|}
%\sum_{t \in T_0}
%Q_{\pi_p}(s_t,a_t)
%\end{equation}
%Compared to the Naive estimator, \eqref{eq:naive}, we see that the estimator takes a remarkably similar form, except that as opposed to an empirical average of rewards, we compute an empirical average of $Q$ values. The idea is that doing so will hopefully compensate for the shift in distribution induced by $\pi_p$. {\em Crucially, we rely on the $Q$-function  corresponding to $\pi_p$}. Since the experiment generates data under this very policy, it tuns out that these $Q$-values are substantially easier to estimate. 
%
%We will return later to the estimation of $Q_{\pi_p}$, saying for now simply that this is a relatively straightforward task, and amenable to a variety of approximation techniques for large state spaces. For now, let us assume we can calculate $Q_{\pi_p}$ and return to Example~\ref{eq:two_state}. 
%
%\begin{example}[Continued] 
%\label{eg:two_state}
%Continuing with our example, we can readily calculate 
%\[
%\begin{split}
%Q_{\pi_p}(\mathbf{0},0) &= - \lambda^{\pi_p} + {1/2}/{(1 - \delta/2)}\\
%Q_{\pi_p}(\mathbf{0},1) &= - \lambda^{\pi_p} + {1/2}/({1 - \delta/2})\\
%Q_{\pi_p}(\mathbf{1},0) &= 1 - \lambda^{\pi_p} + {1/2}/({1 - \delta/2})\\
%Q_{\pi_p}(\mathbf{1},1) &= 1 - \lambda^{\pi_p} + ({1/2 + \delta})/({1 - \delta/2})
%\end{split}
%\] 
%where the average reward under $\pi_p$, $\lambda^{\pi_p} = 1/2/(1-\delta/2)$. Now, for a dataset generated under the stationary distribution corresponding to $\pi_p$, we may trivially calculate
%\[
%\E \left[
%\hat {\rm ATE}_D
%\right]
%= 
%\frac{1}{2} \left(
%\frac{\delta}
%{(1 - \delta/2)^2}
%\right)
%\]
%In other words, the bias in the Dynkin estimate is second-order (i.e. negligible) relative to the {\em ATE}. That is, as we can readily calculate here $|{\rm ATE} - \E \left[
%\hat {\rm ATE}_D
%\right]| = O(\delta^2)$. 
%%In particular, we have 
%%\[
%%\frac{\rm ATE}{\E \left[
%%\hat {\rm ATE}_D
%%\right]} = 1- \delta/2
%%\]
%\end{example}  
%
%Is the dramatic mitigation of bias we see in Example~\ref{eq:two_state} generic? Our first set of results essentially answers this question in the affirmative. In particular, we make the following Assumption:
%
%\begin{assumption}
%[Lipschitz Transitions]
%We assume that the change in distribution over next states under the intervention is Lipschitz in the treatment effect. Specifically, for any state $s \in \Sscr$,  
%\[
%d_{\rm TV}( p(s,1,\cdot), p(s,0,\cdot) ) \leq L \delta 
%\]
%where $L$ is a Lipschitz constant and $\delta$ is the $ATE$.   
%\end{assumption} 
%The above assumption is relatively benign. In particular, the condition is trivially satisfied for the examples in $\cite{}$. Our first result concerns the bias of the Dynkin estimator, which we show is small: 
%
%\begin{assumption}[Mixing time]
%Let $\rho$ be the stationary distribution under $\pi_{p}.$ There exist $C_{m}$ and $\lambda$ such that
%\begin{align*}
%d_{\rm TV} (P^{k}(s, \cdot), \rho) \leq C_{m} \lambda^{k}. 
%\end{align*}
%\end{assumption}
%
%\begin{theorem}
%$$
%\left|{\rm ATE} - \E \left[
%\hat {\rm ATE}_D
%\right]\right| \leq 2 \left(\frac{C_{m}}{1-\lambda}\right)^2 r_{\max} \cdot \delta^2
%$$
%where $r_{\max} := \max_{s,a} r(s,a).$
%\end{theorem}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> Tex Files/Experiments.tex <==
\section{Experiments} \label{sec:experiments}
This section will empirically investigate the DQ estimator and a number of alternatives in two settings: the simple example of Section~\ref{sec:example}, originally
proposed by \cite{johari2022experimental}; and more realistically, a city-scale simulator of a ride-hailing platform similar to what large ride-hailing operators use in production. The alternatives we consider include: 1) the Naive estimator;  2) TSRI-1 and TSRI-2, the ``two-sided randomization'' (TSR) designs/estimators from \cite{johari2022experimental}; and 3) a variety of OPE estimators. For the OPE estimators, we note that off-policy average reward estimation has only recently been addressed in \cite{wanLearningPlanningAverageReward2021,zhangAverageRewardOffPolicyPolicy2021}, and we implement their specific estimators which we simply denote as TD and GTD respectively. We also implement an extension to an LSTD type estimator proposed in \cite{shi2020reinforcement}.
\subsection{A Simple Example}
We first study all of our estimators in the example of Section~\ref{sec:example}, a simple setting that does not call for any sort of value function approximation. Our goal now is to understand the relative merits of practical implementations of these estimators, in terms of their bias and variance.

To recap, this MDP is a stylized model of a rental marketplace, consisting of a 1-D Markov chain on $N=5000$ states parameterized by a `customer arrival' rate $\lambda$ and a `rental duration' rate $\mu$. At a given state $n$ (so that $n$ units of inventory are in the system), the probability that an arriving customer rents a unit is impacted by the intervention. As such if the intervention increases the probability of a customer renting, this reduces the inventory availability for customers that arrive later. Our MDP and experimental setup exactly replicates that of \cite{johari2022experimental}, with $N=5000, \lambda=1, \mu=1$.
\begin{figure}[htbp]
 \centering
 \subfloat{\includegraphics[width=0.46\textwidth]{fig/synthetic-distributions.pdf}}
 \subfloat{\includegraphics[width=0.54\textwidth]{fig/synthetic.pdf}}
 \caption{Toy-example from \cite{johari2022experimental}. {\it Left}: Estimated ATE at time $t/N=10^{4}$ across $100$ trajectories. Dashed line indicates actual ATE. Diamonds indicate the asymptotic mean for each estimator. DQ shows compelling bias-variance tradeoff for this experimental budget.  {\it Right}: Relative RMSE vs. Time; DQ dominates the alternatives at all timescales. }
 \label{fig:birth-death}
\end{figure}
We run all estimators over 100 separate trajectories of length $t=10^{4} N$ of the above MDP initialized in its stationary distribution. Figure~\ref{fig:birth-death} summarizes the results of this experiment. Beginning with the left panel, which reports estimated quantities at $t = 10^4 N$, we immediately see:
\newline
\textbf{TSR improves on Naive: }The actual ATE in the experiment is $1.5\%$. Whereas it has the lowest variance of the estimators here, the Naive estimator has among the highest bias. The two TSR estimators reduce this bias substantially at a modest increase in variance. It is worth noting, as a sanity check, that these results precisely recreate those reported in \cite{johari2022experimental}. 
\newline
\textbf{OPE estimators are high variance: }The OPE estimators have the highest variance of those considered here. The TD estimator has the lower variance but this is simply because it is implicitly regularized. Run long enough, both estimators will recover the treatment effect.  
\newline
\textbf{DQ shows a compelling bias-variance tradeoff: }In contrast, the DQ estimator has the lowest bias at $t = 10^4 N$ and its variance is comparable to the TSR estimators (It is worth noting that run long enough, the DQ estimator had a bias of  $\sim-5 \times 10^{-7}$).
\newline
\textbf{Conclusions hold across experimental budgets: }Turning our attention briefly to the right chart in Figure~\ref{fig:birth-death}, we show the relative RMSE (i.e. RMSE normalized by the treatment effect) of the various estimators considered here {\em across all experimental budgets} $t$. RMSE effectively scalarizes bias and variance and we see that on this scalarization the DQ estimator dominates the other estimators considered here over all choice of $t$.

We note that specialized designs such as TSR can still be valuable in specific settings: when $\lambda \gg \mu$, for example, TSR is nearly unbiased (see \cite{johari2022experimental}), and can outperform DQ; see the appendix for such a study.
\subsection{A Large-Scale Ridesharing Simulator}
We next turn our attention to a city-scale ridesharing simulator similar to those used in production at large ride-hailing services. We will consider the problem of experimenting with changes to {\em dispatching} rules. Experimenting with these changes naturally creates Markovian interference by impacting the downstream supply/ positioning of drivers. Relative to the earlier toy example, the corresponding MDP here has an intractably large state-space, necessitating value function approximation for the DQ and OPE estimators.

%
%\cite{johari2022experimental}
%
%
%\paragraph{Problem setup} We first demonstrate the effectiveness of the Dynkin estimator on a simple, tabular MDP. For this we use the Markov chain from \cite{johari2022experimental}, a stylized model of a two-sided marketplace. Customers arrive at rate $\lambda$ and choose whether to purchase one of $N$ listings, based on a multinomial logit model. Upon purchase, a given listing is removed from the marketplace for an exponentially distributed duration with rate $\mu$, after which it becomes available for purchase again. The intervention is a UI change, which influences customers' purchase probabilities. In the language of MDPs, state is the number of listings available; actions are binary, indicating whether to apply the intervention to a given customer; and rewards are 1 if a customer makes a purchase and 0 otherwise. Customers interfere with each other because they share the same limited pool of listings; for example, increasing the booking rate of the treatment group decreases listings available to the control group. Our experimental setup exactly replicates that of \cite{johari2022experimental}, with $N=5000, \lambda=1, \mu=1$; see the Appendix for further details.
%
%\paragraph{Estimators} We compare several alternatives: 1) the naive estimator; 2) the off-policy estimator from \cite{shi2020reinforcement}; 3) TSRI-1 and TSRI-2, the ``two-sided randomization'' (TSR) estimators from \cite{johari2022experimental}; and 4) the Dynkin estimator . For the Dynkin estimator, we estimate the Q-function via LSTD \cite{konda2002actor}; we describe this implementation in detail in Section~\ref{sec:implementation}. For the off-policy estimator, we note that off-policy average reward estimation has only recently become possible, due to \cite{wanLearningPlanningAverageReward2021,zhangAverageRewardOffPolicyPolicy2021}. We implement these state-of-the-art estimators along with an LSTD variant, which we describe in detail in the Appendix. TSRI-$k$ estimators are allowed to choose the experimental design (both rider-side and driver-side randomization probabilities) as well as the estimator based on the rate parameters $\lambda,\mu$, as prescribed in \cite{johari2022experimental}.
%
%Figure~\ref{fig:birth-death} shows the RMSE of each estimator as a function of time. As demonstrated in \cite{johari2022experimental}, the Naive estimator exhibits low variance but considerable bias. The TSRI estimators mitigate bias through better design and estimation, but ultimately are also low-variance, high bias estimators. The Off-Policy estimator is asymptotically unbiased, but exhibits large variance for the horizons we simulate. Even in this setting, which can be viewed as ``home court'' for the TSRI estimators, the Dynkin estimator exhibits a much more favorable bias-variance tradeoff over all horizons, with bias vanishing as $t$ grows large. In fact the asymptotic bias of the Dykin estimator turns out to be negligible; its theoretical value (according to Theorem~\ref{}) is $-3 \times 10^{-5}$, relative to an effect size of 0.015.



% \begin{table}[htbp]
%   \centering

% \begin{tabular}{clrrrrr}
% \toprule
% ATE & Estimator & $\hat{\mathrm{ATE}}$: Mean ($T=\infty$) & Mean ($T=10^3$) & p10 & p50 & p90\\
% \midrule
% 1.55 & Naive &1.88& 1.88 & 1.85 & 1.89 & 1.91\\
% & DQ &1.55& 1.61 & 1.54 & 1.62 & 1.67\\
% & OPE (LSTD) &1.55& 1.31 & -0.76 & 1.44 & 3.06\\
% & OPE (TD) &1.55& 1.88 & 1.52 & 1.85 & 2.25\\
% & TSRI-1 &1.83& 1.83 & 1.79 & 1.83 & 1.88\\
% & TSRI-2 &1.67& 1.67 & 1.60 & 1.67 & 1.74\\
% \bottomrule
% \end{tabular}

%   \caption{Asymptotic bias, and variance at $t/N = 10^{4}$ for various estimators on the Markov chain from \cite{johari2022experimental}. The Dynkin estimator exhibits by far the smallest bias of the biased estimators, and much lower variance than the unbiased OPE estimators.}
% \end{table}


\textbf{The Simulator: }Ridesharing admits a natural MDP; see e.g. \cite{qinReinforcementLearningRidesharing2021}. The state at the time of a request corresponds to that of all drivers at that time: position, assigned routes, riders, and the pickup/dropoff location of the request. Actions correspond to driver assignments and pricing decisions. The reward for a request is the price paid by the rider, less cost incurred to service the request.
%The problem of choosing a profit-maximizing dispatch policy, for example, can be modeled as an MDP where each time step corresponds to a request; the state is the set of drivers in the system, their assigned routes and riders, and the pickup / dropoff location of the request; actions correspond to dispatch decisions (i.e the assignment of a request to a driver) and 
%pricing, and the reward for each request is the price paid by the rider, less the cost incurred to service the request. 
Our simulator models Manhattan. Riders and drivers are generated according to real world data, based on \cite{TLCTripRecord}; this yields $\sim 300k$ requests and $\sim 7k$ unique drivers per real day. An arriving request is served a menu of options generated by a price engine. The rider chooses an option based on a choice model calibrated on taxi prices (for the outside option) and delay disutility. A dispatch engine assigns a driver to the rider; the engine chooses the driver who can serve the rider at minimal marginal cost, subject to the product's constraints. Finally drivers proceed along their assigned routes until the next request is received. The simulator implements pooling. Users can switch out demand and supply generation, pricing and dispatch algorithms, driver repositioning, and the choice model via a simple API. Other simulators exist in the literature \cite{qinReinforcementLearningRidesharing2021,yaoRidesharingSimulationPlatform2021}, but either lack an open-source implementation, or implement a subset of the functionality here.

\textbf{The Experiment: }We experiment with dispatch policies. Specifically, we consider assigning a request to an idle driver or a `pool' driver, i.e. a driver who already has riders in their car. A dispatch algorithm might prefer the former, but only if the cost of the resulting trip is at most $\alpha \%$ higher than the cost of assigning to a pool driver. We consider three experiments, each of which changes $\alpha$ from a baseline of $0$ to one of three distinct values: $30\%, 50\%$ or $70\%$, with ATEs of 0.5\%, -0.9\%, and -4.6\% respectively. As we noted earlier, we would expect significant interference in this experiment (or indeed any experiment that experiments with pricing or dispatch) since an intervention changes the availability / position of drivers for subsequent requests.

\begin{figure}[htbp]
  \centering
  \subfloat{\includegraphics[width=0.59\textwidth]{fig/rideshare-distributions.pdf}}
  \subfloat{\includegraphics[width=0.41\textwidth]{fig/ridesharing.pdf}}
  \caption{Ridesharing model 
   {\it Left:} $\hat{\mathrm{ATE}}$ at $t = 3\times10^{5}$ over $50$ trajectories. Dashed line indicates actual ATE. DQ has lowest bias, and is only estimator to estimate correct sign of the treatment at all effect sizes.
  {\it Right:} RMSE vs. Time; DQ dominates at all time scales. 
  }
 \label{fig:rideshare}
\end{figure}

Figure~\ref{fig:rideshare} summarizes the results of the above experiments, wherein each estimator was run over $50$ independent simulator trajectories, each over $3\times10^5$ requests. The DQ and OPE estimators shared a common linear approximation architecture with basis functions that count the number of drivers at every occupancy level. We note that this approximation introduces its own bias which is not addressed by our theory. We immediately see: 
\newline
\textbf{Strong Impact of Interference: }As we might expect, interference has a significant impact here as witnessed by the large bias in the Naive estimator. 
\newline
\textbf{Incumbent estimators do not improve on Naive: }None of the incumbent estimators improve on Naive in this hard problem. This is also the case for the TSR designs, which in this large scale setting surprisingly appear to have significant variance. The OPE estimators have lower variance due to the regularization caused by value function approximation.
\newline
\textbf{DQ works: }In all three experiments, the bias in DQ (although in a relative sense higher than in the toy model) is {\em substantially} smaller than the alternatives, and also smaller than the ATE. This is evident in the left panel in Figure~\ref{fig:rideshare}. Notice that in the rightmost experiment (ATE $= 0.5$), DQ is the only estimator to learn that the ATE is positive. Like in the toy model, the right panel shows that these results are robust over experimentation budgets.  

%The actual ATE in the experiment is $1.5\%$. Whereas it has the lowest variance of the estimators here, the Naive estimator has among the highest bias. The two TSR estimators reduce this bias substantially at a modest increase in variance. It is worth noting that these results precisely recreate those reported in \cite{johari2022experimental}. 
%\newline
%\textbf{OPE estimators are high variance: }The OPE estimators have the highest variance of those considered here. The TD estimator has the lower variance but this is simply because it is implicitly regularized. Run long enough, both estimators will recover the treatment effect.  
%\newline
%\textbf{DQ shows a compelling bias-variance tradeoff: }In contrast, the DQ estimator has the lowest bias at $t = 10^3 N$ and its variance is comparable to the TSR estimators (It is worth noting that run long enough, the DQ estimator had a bias of  $\sim-3 \times 10^{-5}$). 
%\newline
%\textbf{Conclusions hold across experimental budgets: }Turning our attention briefly to the right chart in Figure~\ref{fig:birth-death}, we show the relative RMSE (i.e. RMSE normalized by the treatment effect) of the various estimators considered here {\em across all experimental budgets} $t$. RMSE effectively scalarzies bias and variance and we see that on this scalarization the DQ estimator dominates the other estimators considered here over all choice of $t$. 



 
% Beginning with the left panel, which reports estimated quantities at $t = 10^3 N$, we immediately see: 
%
%
%In ridesharing applications, a common goal is to evaluate the impact of a change in the dispatch algorithm on profits, for example. We describe one specific intervention of this type below.
%
% Riders may be dispatched either to an idle driver, or to a ``pool'' driver, i.e. a driver who already has riders in their car. A pool driver can often serve a rider at lower marginal cost than an idle driver, by adding the rider to their existing route. However, doing so reduces the pool driver's flexibility to serve future riders, and can thereby increase costs in the long term. As a heuristic to manage this tradeoff between short-term and long-term rewards, the platform can preferentially dispatch idle drivers. Specifically, the platform will dispatch an idle driver if the cost is up to $\alpha$\% higher than the minimum cost driver. In control, we set this threshold to be $\alpha_{\rm co} = 0$; in treatment, we test various thresholds $\alpha_{\rm tr}$.
%
%Our approach to experimentation here is rider-level randomization: for each rider, choose control or treatment at random, and select the minimum cost driver satisfying the threshold. Note that the naive difference-in-means estimator here will entirely fail to capture the long-term effects of each policy. More generally, ``interference'' in rider-level experiments occurs because all riders share the same supply of drivers; each dispatch decision changes the state of this shared supply; and therefore the treatment assignment for the $t^{\rm th}$ rider may affect outcomes for future riders regardless of whether they are assigned control or treatment. Virtually any rider-level experiment on a ridesharing platform -- pricing, dispatch, or otherwise -- may alter the state of supply and therefore induce Markovian interference.
%
%
%%Broadly, the simulator's dynamics are as follows: 1) Riders and drivers are generated based on real world data \cite{}; 2) a pricing engine offers a menu of prices and products (typically, different levels of convenience) to the rider; 3) the rider selects a product from this menu according to their choice model; 3) a dispatch engine decides which driver to assign to the rider; by default, we choose the driver who can serve the rider at minimal marginal cost, subject to the product's constraints; and 4) drivers proceed along their assigned routes until the next request is received. The simulator implements pooling, where a driver can serve multiple riders concurrently.
%%
%%The simulator interfaces with each generative model or algorithm via a simple API. This gives the modeler modular control over demand and supply generation, pricing and dispatch algorithms, driver repositioning, and the rider choice model. Pricing and dispatch policies may depend on the entire system state. We also provide a framework for A/B testing with the pricing and dispatch engines, and two-sided experimentation (as in \cite{johari2022experimental}) for the dispatch engine.
%%
%%A variety of simulators exist in the literature, but most either lack an open-source implementation, or implement only a subset of the functionality we describe here. See  \cite{qinReinforcementLearningRidesharing2021,yaoRidesharingSimulationPlatform2021} for surveys of alternatives.
%
%\subsection{Ridesharing experiments and interference}
%
%In ridesharing applications, a common goal is to evaluate the impact of a change in the dispatch algorithm on profits, for example. We describe one specific intervention of this type below.
%
%Riders may be dispatched either to an idle driver, or to a ``pool'' driver, i.e. a driver who already has riders in their car. A pool driver can often serve a rider at lower marginal cost than an idle driver, by adding the rider to their existing route. However, doing so reduces the pool driver's flexibility to serve future riders, and can thereby increase costs in the long term. As a heuristic to manage this tradeoff between short-term and long-term rewards, the platform can preferentially dispatch idle drivers. Specifically, the platform will dispatch an idle driver if the cost is up to $\alpha$\% higher than the minimum cost driver. In control, we set this threshold to be $\alpha_{\rm co} = 0$; in treatment, we test various thresholds $\alpha_{\rm tr}$.
%
%Our approach to experimentation here is rider-level randomization: for each rider, choose control or treatment at random, and select the minimum cost driver satisfying the threshold. Note that the naive difference-in-means estimator here will entirely fail to capture the long-term effects of each policy. More generally, ``interference'' in rider-level experiments occurs because all riders share the same supply of drivers; each dispatch decision changes the state of this shared supply; and therefore the treatment assignment for the $t^{\rm th}$ rider may affect outcomes for future riders regardless of whether they are assigned control or treatment. Virtually any rider-level experiment on a ridesharing platform -- pricing, dispatch, or otherwise -- may alter the state of supply and therefore induce Markovian interference.
%
%Following \cite{johari2022experimental,bajariMultipleRandomizationDesigns2021}, we can also implement two-sided randomization to test this intervention. That is, we randomize riders and drivers into treatment and control. Untreated riders are dispatched to the minimum cost driver satisfying threshold $\alpha_{\rm co}$, while treated riders are dispatched to the minimum cost driver, among {\it treated} pool drivers satisfying threshold $\alpha_{\rm tr}$ and {\it control} pool drivers satisfying threshold  $\alpha_{\rm co}$. Note that this type of two-sided randomization is specific to this intervention -- many other ridesharing experiments, such as pricing experiments, suffer from Markovian interference but have no natural implementation of two sided randomization.
%
%\subsection{Results}
%
%% We compare the the following estimators: 1) The Dynkin estimator; 2) the naive estimator; 3) the off-policy estimator of \cite{shi2020reinforcement}; and 4) the two-sided randomization estimators TSRI-1 and TSRI-2 of \cite{johari2022experimental}. All but the TSRI estimators use data collected according to a rider-side randomization scheme. The Dynkin estimator estimates the Q-functions via LSTD with linear function approximation, using a set of features which describe the request and the state of supply. The Off-Policy estimators use the same set of features, using the state-of-the-art TD (\cite{wanLearningPlanningAverageReward2021}), GTD (\cite{zhangAverageRewardOffPolicyPolicy2021}), or LSTD estimators of the off-policy average reward. The two-sided randomization probabilities for TSRI-1 and TSRI-2, as well as the estimator hyperparameters, are set based on average demand arrival rates and service times as prescribed in \cite{johari2022experimental}. See the Appendix for further implementation details.
%
%% The LSTD off-policy estimator initially suffers from large variance, although it eventually attains performance comparable to the naive estimator; the function approximation likely helps to reduce variance here at the cost of bias. Performance for the TD and GTD Off-Policy estimators is initially good, but the estimators eventually converge to performance similar to the Naive estimator. The TSRI-$k$ estimators are dominated by Naive throughout, although they ultimately attain a comparable RMSE. While \cite{johari2022experimental} shows that these estimators are unbiased when the system is extremely supply constrained or demand constrained, in the realistic regime we simulate they appear to provide little benefit. The Dynkin estimator dominates the alternatives throughout in terms of RMSE.
%
%
%\begin{figure}[htbp]
%  \centering
%  \subfloat{\includegraphics[width=0.41\textwidth]{fig/ridesharing.pdf}}
%  \subfloat{\includegraphics[width=0.59\textwidth]{fig/rideshare-distributions.pdf}}
%  \caption{Performance of various estimators on the ridesharing intervention, for varying ATEs. {\it Left:} RMSE vs. time, on the intervention with an ATE of -4.6\%. {\it Right:} Distribution of $\hat{\mathrm{ATE}}$ for each estimator for each effect size, at $t = 3 \times 10^{5}$. Dashed line indicates actual ATE. DQ attains low bias and variance throughout, and is the only estimator to correctly estimate the sign of the treatment at all effect sizes.}
% \label{fig:rideshare}
%\end{figure}


% \begin{table}[htbp]
%   \centering
% \begin{tabular}{rlrrrr}
% \toprule
% ATE & Estimator & $\hat{\mathrm{ATE}}$: Mean & p90 & p50 & p10\\
% \midrule
% 0.5 & Dynkin & 1.0 & 1.4 & 1.0 & 0.8\\
%  & Naive & -1.5 & -1.2 & -1.5 & -1.7\\
%  & Off-Policy (GTD) & -1.3 & -0.6 & -1.5 & -1.8\\
%  & Off-Policy (LSTD) & -1.5 & -0.9 & -1.6 & -1.9\\
%  & Off-Policy (TD) & -1.4 & -0.9 & -1.4 & -1.9\\
%  & TSRI1 & -2.6 & -2.6 & -2.6 & -2.6\\
%  & TSRI2 & -2.9 & -2.9 & -2.9 & -2.9\\
%   \hline
% -0.9 & Dynkin & -1.8 & -1.6 & -1.8 & -2.2\\
%  & Naive & -4.2 & -3.9 & -4.2 & -4.4\\
%  & Off-Policy (GTD) & -4.1 & -3.8 & -4.2 & -4.5\\
%  & Off-Policy (LSTD) & -4.2 & -3.8 & -4.1 & -4.6\\
%  & Off-Policy (TD) & -4.2 & -3.7 & -4.1 & -4.7\\
%  & TSRI1 & -4.3 & -3.5 & -4.1 & -5.1\\
%  & TSRI2 & -4.9 & -4.0 & -4.6 & -6.1\\
%   \hline
% -4.6 & Dynkin & -5.9 & -5.4 & -6.0 & -6.3\\
%  & Naive & -8.4 & -8.2 & -8.3 & -8.7\\
%  & Off-Policy (GTD) & -8.4 & -8.0 & -8.4 & -8.7\\
%  & Off-Policy (LSTD) & -8.3 & -7.9 & -8.3 & -8.7\\
%  & Off-Policy (TD) & -8.3 & -7.9 & -8.3 & -8.6\\
%  & TSRI1 & -8.4 & -7.5 & -8.5 & -8.9\\
%  & TSRI2 & -9.2 & -8.3 & -9.4 & -10.0\\
% \bottomrule
% \end{tabular}

% \caption{RMSE of various estimators, over different effect sizes and timescales (measured in the number of requests). The Dynkin estimator exhibits the lowest RMSE of any estimator, over all timescales.}
% \end{table}

% 2a. Pricing

% - Experiment
% - Type of interference
% - Type of designs

% 2b. Dispatch

% 3. Results
% 3a. Naive does not work. (bias is large)
% 3b. Dominate the alternatives.
% 3c. Great alternative to switchbacks.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> Tex Files/Interpolation.tex <==
\section{Discussion: Bias-Variance Tradeoffs, Policy Optimization} \label{sec:conclusion}

To summarize, we have shown that the DQ estimator achieves a surprising bias-variance tradeoff by applying on-policy estimation to the Markovian interference problem, and more generally to OPE. Here we draw further connections between the Naive, DQ, and OPE estimators and provide methods to realize other points on the bias-variance curve. Furthermore, we draw surprising connections between our estimator and trust-region methods in policy optimization, and show that DQ can serve as a drop-in replacement for these policy optimization surrogates with {\it  provably} lower bias.

\subsection{A $k^{\rm th}$-order Bias Correction}\label{sec:korder-correction}

As alluded to in Section~\ref{sec:estimator}, we can view the DQ estimator as a first-order correction to the Naive estimator, based on a Taylor series expansion of the ATE. This immediately motivates a $k^{\rm th}$-order correction, with the goal of obtaining estimators with bias $O(\delta^{k+1})$ for arbitrary $k$.

This correction turns out to have a suprising and intuitive form\footnote{For now, we assume for simplicity that rewards are only a function of state. Similar results can be derived for the more general case where $r$ is a function of both state and action, although the resulting formulas are more complex}. In short, to obtain the $k^{\rm th}$ order correction term for $k$ odd (the correction for $k$ even is 0), we simply compute the DQ estimator, but replace rewards in the MDP with the $(k-1)^{\rm th}$ order Difference-in-Q functions -- effectively a Difference-in-Qs-of-Difference-in-Qs.

Precisely, for some reward function $f: \mathcal{S} \mapsto \mathbb{R}$, we can define an auxiliary MDP with the same transition  probabilities, but rewards $f(s)$ at each state. Let $Q(s, a; f)$ be the corresponding Q function, under policy $\pi_{1 / 2}$. We now define
the $k^{\rm th}$ order Q-function to be $Q^{(k)}(s, a) = Q(s, a; f^{(k-1)})$, where the rewards are defined as $f^{(k-1)}(s) = \frac{1}{2} \left( Q^{(k-1)}(s, 1) - Q^{(k-1)}(s, 0) \right)$; in other words, the previous-order Difference-in-Q functions. We take as a base case $f^{(0)}(s) = r(s)$. Finally, we can define the $K^{\rm th}$-order Difference-in-Qs estimate of the ATE to be the sum of all lower-order correction terms: $
\hat{\mathrm{ATE}}_{\rm DQ}^{(K)} = \sum_{k \text{ odd}, k \leq K} \mathbb{E}_{\rho_{1/2}}\left[Q^{(k)}(s, 1) - Q^{(k)}(s, 0)\right]$.

In principle this approach enables {\it off-policy}  evaluation with arbitarily low bias -- entirely via estimation of {\it on-policy} quantities. One can verify that ${\rm{ATE}}_{\rm DQ}^{(1)}$ is the expected value of the DQ estimator. We now generalize \cref{th:dynkin_bias} to provide a bias bound for the $k^{\rm th}$ order correction\footnote{The variance of such plug-in estimators can be bounded by iteratively applying \cref{lem:non-expansive-lemma}, which is omitted for simplicity.}:

\begin{theorem}\label{th:korder-bias}
For any $K=0, 1, 2, \dotsc$, we have $\left|{\rm{ATE}} - {\rm{ATE}}_{\rm DQ}^{(K)}\right| \leq C' \left(\frac{1}{1-\lambda}\right)^{K+1} \delta^{K+1} r_{\max}$, where $C'$ is a constant depending (polynomially) on $\log(C).$
\end{theorem}
% We can use the plug-in empirical estimator for ${\rm{ATE}}_{\rm DQ}^{(K)}.$ The variance for such an estimator can be bounded by iteratively applying \cref{lem:non-expansive-lemma}. We will leave the explicit form for the bounds to the future work.
% \textbf{Difference-in-Q iterations.} Roughly speaking, for achieving an $O(\delta^{k})$ bias, the idea is to \textit{iteratively} compute difference-in-Q functions for $k$ iterations. That is,


% At each iteration, the difference in Q functions from the previous iteration is viewed as a \textit{new reward function} and then the new $Q$-function (as well as the new difference-in-Q function) can be computed based on this reward function.

% In particular, let $r^{(0)}_{+}(\cdot, 0) = r^{(0)}_{+}(\cdot, 1) = r(\cdot, 1)$ and $Q^{(0)}_{+}$ be the associated $Q$-value function of $r^{(0)}_{+}$ (all $Q$-value functions are computed under the policy $\pi_{1/2}$ if not mentioned otherwise). Then for $k \geq 1$, Let $Q^{(k)}_{+}$ be the $Q$-value functions corresponding to the rewards $r^{(k)}_{+}$ where
% \begin{align*}
% r^{(k)}_{+}(\cdot, 0) = r^{(k)}_{+}(\cdot, 1) := \frac{Q^{(k-1)}_{+}(\cdot, 1) - Q^{(k-1)}_{+}(\cdot, 0)}{2}
% \end{align*}
% i.e., we assign the rewards at the $k$th iteration to be the difference in the $Q$-value function at the $(k-1)$th iteration.

% Similarly, let $r^{(0)}_{-}(\cdot, 0) = r^{(0)}_{-}(\cdot, 1) = r(\cdot, 0)$ and $Q^{(0)}_{-}$ be the associated $Q$-value function of $r^{(0)}_{-}$. For $k\geq 1$, let $Q^{(k)}_{-}$ be the $Q$-value functions corresponding to the rewards $r^{(k)}_{-}$ where
% \begin{align*}
% r^{(k)}_{-}(\cdot, 0) = r^{(k)}_{-}(\cdot, 1) := \frac{Q^{(k-1)}_{-}(\cdot, 0) - Q^{(k-1)}_{-}(\cdot, 1)}{2}.
% \end{align*}

% We then define the following quantity that corrects the $K$th-order bias.
% \begin{align*}
% {\rm{ATE}}_{\rm DQ}^{(K)} := \sum_{k=0}^{K} \left[\sum_{s} \rho_{1/2}(s) \left( r^{(k)}_{+}(s, 1) - r^{(k)}_{-}(s, 0)\right)\right].
% \end{align*}

\subsection{Interpolating from OPE to Naive via Regularization}

Here, we view the DQ estimator again as an intermediate point on the bias-variance curve between Naive and OPE. This time, however, we interpolate between these extremes by regularizing certain key nuisance parameters in estimating the ATE.

\paragraph{An OPE meta-estimator.} First, we situate the DQ estimator in the context of existing OPE techniques. Consider the following exact identity for the ATE:  $\mathrm{ATE} = \E_{\rho_{1 / 2}}[\zeta(s) (Q_{\pi_{1 / 2}}(s, 1) - Q_{\pi_{1 / 2}}(s, 0))]$ where $\zeta(s) = \frac{1}{2}\frac{ \rho_{1}(s) + \rho_{0}(s)}{\rho_{1 / 2}(s)}$ is the likelihood ratio of the stationary distributions. A variety of OPE estimators -- including doubly-robust (\cite{kallus2020double,ueharaMinimaxWeightQFunction2020}) and primal-dual (\cite{daiBoostingActorDual2017,tangDoublyRobustBias2019}) estimators -- in fact estimate ATE explicitly by plugging in estimates $\hat{\zeta}, \hat{Q}_{\pi_{1 / 2}}$ of the likelihood ratio and value functions (referred to as the ``doubly-robust meta-estimator'' in \cite{kallus2020double}):

\begin{equation}
  \label{eq:dr-meta}
 \hat{\mathrm{ATE}}_{\rm DR} = \frac{1}{|T_{1}|}\sum_{t \in T_1}\hat{\zeta}(s_t) \hat{Q}_{\pi_{1 / 2}}(s_t, 1) - \frac{1}{|T_0|} \sum_{t\in T_0}\hat{\zeta}(s_t) \hat{Q}_{\pi_{1 / 2}}(s_t, 0)
\end{equation}
%\paragraph{Refining the Bias-Variance Tradeoff.} Immediately, we see that that by taking the likelihood ratio to be a constant $\hat{\zeta}(s) = 1 \; \forall s$, we recover the DQ estimator $\hat{\mathrm{ATE}}_{\rm DQ}$. Furthermore, if we then take  $\hat{V}_{\pi_{1 / 2}}$ to be any constant $\hat{V}_{\pi_{1 / 2}}(s) = c \; \forall s$, we recover the Naive estimator\footnote{To see this, observe that $\hat{Q}_{\pi_{1 / 2}}(s, a) = r(s, a) + \E \left[\hat{V}_{\pi_{1 / 2}}(s') | s, a\right] = r(s, a) + c$}. The DQ and Naive estimators' relationship to OPE then becomes clear: we obtain DQ by choosing a minimal variance (but highly biased) estimator of $\zeta$; and we obtain the Naive estimator by subsequently choosing a minimal variance (but highly biased) estimator of $V$. This suggests that we can interpolate between these extremes by making more refined bias-variance tradeoffs in estimating $\hat{\zeta}$ and $V_{\pi_{1 / 2}}$. It turns out that several natural approaches to variance reduction provide exactly such an interpolation.

\noindent\textbf{\textsf{Explicit regularization}.} In estimating $\hat{\zeta}(s)$, one can directly penalize its deviation from one, where increasing the penalty interpolates from OPE to DQ. Given that estimation of $\hat{\zeta}(s)$ is the key difference between DQ and unbiased OPE -- and therefore the source of the massive variance gap (Theorems~\ref{th:dynkin_var} and \ref{th:cramer-rao}) -- we would expect this to be a particularly powerful approach to OPE, and indeed similar penalties have produced strong empirical performance \cite{nachum2019dualdice}. Similarly, one can directly penalize the deviation of $\hat{V}_{\pi_{1 / 2}}$ from zero, as in regularized variants of LSTD (see e.g. \cite{kolterRegularizationFeatureSelection2009}). As we increase the regularization penalty on $\hat{\zeta}(s)$, we interpolate from OPE to DQ; additionally increasing the regularization penalty on $\hat{V}_{\pi_{1 / 2}}$ then interpolates from DQ to Naive. Approaches combining both forms of regularization have been explored in \cite{yangOffPolicyEvaluationRegularized2020}.

\noindent\textbf{\textsf{Function approximation}.} More generally, one can restrict $\hat{\zeta}(s)$ and $\hat{V}_{\pi_{1 / 2}}$ to lie in particular function classes, with one extreme being any mapping $\mathcal{S} \mapsto \mathbb{R}$, and the other extreme being the constant functions $\hat{V}_{\pi_{1 /2}}(s) = c$ or $\hat{\zeta}(s) = 1$. As one example, when the state space is massive we may approximate it using state aggregation. At the extreme, aggregating all states into a single aggregate state implies that the value function (or likelihood ratio) must be a constant. As the aggregation for $\hat{\zeta}(s)$ goes from fine to coarse, we  interpolate between OPE and DQ; increasing the coarseness of $\hat{V}_{\pi_{1 / 2}}(s)$ then interpolates between DQ and Naive.
%
%{\bf Discounting.} A common technique to estimate the average reward value function is to instead estimate a  discounted reward value function $Q_{\gamma}(s, a) = \mathbb{E}\left[\sum_{t=0}^T \gamma^{t} r(s_t, a_t) | s_{0} = s, a_0 = a\right]$, motivated by the fact that we obtain exactly the average-reward value function $Q$ as the discount rate $\gamma$ goes to one (under the proper scaling \cite{putermanMarkovDecisionProcesses2014}). Implementing DQ with $\hat{Q}_{\pi_{1 / 2}}(s, a) = (1 - \gamma)Q_{\gamma}(s,a)$ yields the exact DQ estimator as $\gamma \to 1$, and the Naive estimator as $\gamma \to 0$.

\subsection{DQ as a Policy Optimization Objective}
\label{sec:policy-optimization}

\paragraph{Surrogate objectives in trust-region methods}
DQ also has a suprising relationship to trust-region methods \cite{schulman2015trust,schulman2017proximal,kakade2002approximately}. At each iteration, these methods essentially solve an {\it offline} policy optimization problem: using data collected under some ``behavioral''policy $\pi_{\rm b}$, they evaluate (and subsequently optimize) a candidate policy $\pi$. The policy evaluation step is exactly an OPE problem, and they construct a surrogate objective based on an identity sometimes referred to as Dynkin's identity \cite{dynkin1965markov}: $\lambda({\pi}) = \E_{\pi_{b}}[r(s, a)] + \E_{s \sim \rho_{\pi_{b}}, a \sim \pi}\left[ \frac{\rho_{\pi}(s)}{\rho_{\pi_{b}}(s)} \left( Q^{\pi_{b}}(s, a) - V^{\pi_{b}}(s) \right) \right]$, where $\rho_{\pi_b}, V^{\pi_b}, Q^{\pi_b}$ is the stationary distribution, $V$-function, and $Q$-function of the policy $\pi_{b}$ respectively and $\rho_{\pi}$ is the stationary distribution of $\pi$. The referenced trust-region methods then effectively take the likelihood ratio $\rho_{\pi}(s) / \rho_{\pi_{b}}(s)$ to be identically one, yielding the (idealized) surrogate objective:
$\hat{\lambda}_{\rm TR}({\pi}) = \E_{\pi_{b}}[r(s, a)] + \E_{s \sim \rho_{\pi_{b}}, a \sim \pi}\left[  Q^{\pi_{b}}(s, a) - V^{\pi_{b}}(s) \right]$.

\paragraph{A DQ-based surrogate} As it turns out, DQ derives from a very similar identity -- with a small but critical difference which allows DQ to obtain \textit{even lower bias}. Applying the peturbation bound in \cref{lem:perturbation-stationary-distribution} to $\lambda(\pi)$, we obtain a slightly different identity for $\lambda(\pi)$: $\lambda({\pi}) = \E_{\pi_{b}}[r_{\pi}(s)] + \E_{s \sim \rho_{\pi_{b}}, a \sim \pi}\left[ \frac{\rho_{\pi}(s)}{\rho_{\pi_{b}}(s)} \left( Q^{\pi_{b}}(s, a; r_{\pi}) - V^{\pi_{b}}(s; r_{\pi})\right) \right]$ where $r_{\pi}(s) = \mathbb{E}_{a \sim \pi}\left[r(s, a)\right]$ is the expected reward under $\pi$, and recall that $Q^{\pi_{b}}(\cdot, \cdot; r_{\pi}), V^{\pi_{b}}(\cdot, \cdot; r_{\pi})$ are the value functions for an auxiliary MDP with the same transition probabilities, but {\it taking $r_{\pi}$ to be the reward function}. The biased  form of this estimator, which forms the basis of the DQ estimator\footnote{The DQ estimator in our original setting can actually be derived as either $\hat{\lambda}_{\rm TR}(\pi_{1}) -\hat{\lambda}_{\rm TR}(\pi_{0}) $ or $\hat{\lambda}_{\rm DQ}(\pi_{1}) -\hat{\lambda}_{\rm DQ}(\pi_{0}) $, but this results from a very suprising cancellation of terms in the subtraction; i.e. $\hat{\lambda}_{\rm TR}(\pi) $ and $\hat{\lambda}_{\rm DQ}(\pi)$ are individually different estimators with very different properties, as we will see; and the higher-order corrections must be derived from $\hat{\lambda}_{\rm DQ}$.}, is: $\hat{\lambda}_{\rm DQ}({\pi}) = \E_{\pi_{b}}[r_{\pi}(s)] + \E_{s \sim \rho_{\pi_{b}}, a \sim \pi}\left[   Q^{\pi_{b}}(s, a; r_{\pi}) - V^{\pi_{b}}(s; r_{\pi}) \right]$
which is precisely $\hat{\lambda}_{\rm TR}(\pi)$, but computed on an MDP with rewards $r_{\pi}$.
\paragraph{Lower-order bias} This striking resemblance between the surrogatees $\hat{\lambda}_{\rm DQ}(\pi)$ and $\hat{\lambda}_{\rm TR}(\pi)$ naturally raises the question of how they compare. As it turns out, the simple act of replacing the rewards with $r_{\pi}$ in $\hat{\lambda}_{\rm DQ}$ has significant consequences in terms of bias:

\begin{theorem}[Bias of the DQ surrogate] Suppose it holds that $d_{\rm{TV}}(p(s, a, \cdot), p(s, a', \cdot)) \leq \delta $  for all $s, a, a'$, and that $d_{\rm{TV}}(\pi(s, \cdot), \pi'(s, \cdot)) \leq \delta'$ for all $s$. Then, the biases of $\hat{\lambda}_{\rm TR}(\pi)$\footnote{This result for $\hat{\lambda}_{\rm TR}$ is in fact a slightly refined version of the key perturbation bound in \cite{schulman2015trust}.} and $\hat{\lambda}_{\rm DQ}(\pi)$ satisfy
  \begin{align*}
    |\hat{\lambda}_{\rm TR}(\pi) - \lambda^\pi| = O(\delta (\delta')^2 ) && |\hat{\lambda}_{\rm DQ}(\pi) - \lambda^\pi| = O((\delta\delta')^2 )
  \end{align*}
\end{theorem}

This characterization is sharp, in that there exist non-pathological examples where the exact bias of $\hat{\lambda}_{\rm DQ}$ is a factor $\delta$ smaller than that of $\hat{\lambda}_{\rm TR}$. Crucially, this means that even if the distance between {\it policies} has no non-vacuous upper bound (i.e. $\delta' = 2$), as long as the resulting {\it transition functions} are similar, then the bias of $\hat{\lambda}_{\rm DQ}$ will be small, whereas the bias of $\hat{\lambda}_{\rm TR}$ can be of the order of $\delta$. This immediately suggests that optimizing $\hat{\lambda}_{\rm DQ}$ with respect to $\pi$ should allow for both larger and more accurate policy improvement steps.

% The analysis and framework we provide immediately sets the stage for several additional extensions to this idea. First, our bias characterization can be used to penalize estimators of $\hat{\lambda}_{\rm DQ}$ such that they are conservative in  expectation, as in \cite{schulman2015trust,kakade2002approximately}. Unlike these methods, we provide tools to additionally characterize the variance of such estimators, which can then be used to ensure pessimism (or optimism) with high probability, as in (e.g. \cite{thomas2015high}). Finally, the $k^{\rm th}$ order expansion and other regularization techniques discussed above provide levers which can potentially trade off bias and variance optimally in constructing the policy optimization surrogate.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> Tex Files/Introduction.tex <==
\section{Introduction}

Experimentation is a broadly-deployed learning tool in online commerce that is simple to execute, in principle: apply the treatment in question at random (e.g.~an A/B test), and `naively' infer the average effect of the treatment by differencing the average outcomes under treatment and control. About a decade ago, Blake and Coey \cite{blake2014marketplace} pointed out a challenge in such experimentation on Ebay:

\vspace{1em}

\noindent {\em ``Consider the example of testing a new search engine ranking algorithm which steers test buyers towards a particular class of items for sale. If test users buy up those items, the supply available to the control users declines.''}  

\vspace{1em}

\noindent This violation of the so-called Stable Unit Treatment Value Assumption (SUTVA) \cite{cox1958planning} has been viewed as problematic in online platforms as early as Reiley's seminal `Magic on the Internet' work \cite{lucking-reileyUsingFieldExperiments1999}. Blake and Coey \cite{blake2014marketplace} were simply pointing out that the resulting inferential biases were large, which is particularly problematic since treatment effects in this context are typically tiny. The {\em interference} problem above is germane to experimentation on commerce platforms where interventions on a given experimental unit impact other units, since all units share a common inventory of `demand'  or `supply' depending on context.

Despite the ubiquity of such interference, a practical solution is far from settled. An ongoing line of work addresses the problem via {\em experimental design}, assigning treatments carefully to mitigate the bias of `naively'-derived estimators. In the best cases such designs provably reduce bias by exploiting certain application specific structures, but often it is unclear whether the problem at hand affords such structure (a case in point being the search-engine example above, as will be apparent later). As such, experimentation on online platforms still largely relies on simple randomization, i.e.~A/B tests. Motivated by this fact, we focus instead on {\em designing effective  estimators} assuming simple randomization. We demonstrate a novel estimator which, thanks to an effective bias-variance tradeoff, is a compelling alternative to both alternative state-of-the-art estimators as well as bespoke experimental designs when they apply. 

%\vspace{-1em}
\paragraph{Markovian Interference and Existing Approaches:} We study a generic experimentation problem within a system represented as a Markov Decision Process (MDP), where treatment corresponds to an action which may interfere with state transitions. This form of interference, which we refer to as {\em Markovian}, naturally subsumes the platform examples above, as recently noted by others either implicitly \cite{qinReinforcementLearningRidesharing2021} or explicitly \cite{johari2022experimental,shi2020reinforcement}. In that example, a user arrives at each time step, the platform chooses an action (whether to treat the user), and the user's purchase decision alters the system state (inventory levels).

Our goal is to estimate the Average Treatment Effect (ATE), defined as the difference in steady-state reward with and without applying the treatment. In light of the above discussion, we assume that experimentation is done under simple randomization (i.e.~A/B testing). Now without design as a lever, there are perhaps two existing families of estimators:
\newline
\textbf{1. Naive:} We will explicitly define the {\em Naive} estimator in the next section, but the strategy amounts to simply ignoring the presence of interference. This is by and large what is done in practice. Of course it may suffer from high bias (we show this momentarily in Section~\ref{sec:example}), but it serves as more than just a strawman. In particular, bias is only one side of the estimation coin, and with respect to the other side, namely variance, the Naive estimator is effectively the best possible.
\newline
\textbf{2. Off-Policy Evaluation (OPE):} Another approach comes from viewing our problem as one of policy evaluation in reinforcement learning (RL). Succinctly, it can be viewed as estimating the average reward of two different policies (no treatment, or treatment) given observations from some {\em third} policy (simple randomization). This immediately suggests framing the problem as one of {\em Off-Policy Evaluation}, and borrowing one of many existing {\em unbiased} estimators, e.g.~\cite{thomas2015high,thomas2016data,liu2018breaking,jiang2016doubly,kallus2020double,kallus2022efficiently}. This tack appears to be promising, e.g.~\cite{shi2020reinforcement}, but we observe that the resulting variance is necessarily large ({\bf Theorem \ref{th:cramer-rao}}).
%State-of the-art estimators for this problem proposed in recent years attempt to heuristically correct for the interference between experimental units and thus mitigate bias. But the extent to which these estimators mitigate the problem at hand is largely only understood experimentally. The problem at hand is a hard one since real-world experiments with such interference often have limited experimentation budgets, which ends up ruling out more sophisticated estimators due to their variance.

%\vspace{-1em}
\paragraph{Our Contributions:}
%This paper seeks to construct a practical solution to the problem of inference in experiments with Markovian interference. We do so by viewing the problem at hand as one of policy evaluation in reinforcement learning (RL). Succinctly, the mathematical task implicit in our problem can be viewed as estimating the difference in the average reward of a {Markov Decision Process} (MDP) under one of two policies corresponding to whether or not the intervention is implemented. This difference is in essence the so-called Average Treatment Effect (ATE) of the intervention. The challenge is that we must estimate the ATE given observations from some {\em third} policy corresponding to the experimental design employed. This immediately suggests using ideas from Off-Policy Evaluation to construct unbiased estimators of the ATE. Disappointingly, we observe that while such estimators are unbiased, their variance is substantially larger than incumbent state-of-the art heuristics.
Against the above backdrop, we propose a novel {\em on}-policy treatment-effect estimator, which we dub the `Differences-In-Q's' (DQ) estimator, %\footnote{The name is a nod to a theorem of \cite{dynkin1965markov} that is oft-used (though rarely cited) in the control literature.}
for experiments with Markovian interference. In a nutshell, we characterize our contribution as follows:

\noindent {\em The DQ estimator has provably negligible bias relative to the treatment effect. Its variance can, in general be exponentially smaller than that of an efficent off-policy estimator. In both stylized and large-scale real-world models, it dominates state-of-the-art alternatives}.

We next describe these relative merits in greater detail:
\newline
\textbf{1. Second-order Bias: }We show ({\bf Theorem \ref{th:dynkin_bias}}) that when the impact of an intervention on transition probabilities is $O(\delta)$, the bias of the DQ estimator is $O(\delta^2)$. The DQ estimator thus leverages the one piece of structure we have relative to generic off-policy evaluation: treatment effects are typically small. Our analysis introduces a novel Taylor-like expansion of the ATE (Theorem~\ref{th:korder-bias}) that in addition to the current setting, is of general interest in the theory of RL (for instance, in the context of Policy Optimization). 
% wherein the suppressed constants depend {\em logarithmically} on the size of the state space.
%One approach to dealing with the challenge above is collecting a sufficient amount of data under the design policy so as to effectively reconstruct the steady state distribution under both the intervention and no-intervention policies. This is `off policy' estimation and while unbiased, it typically requires a large number of observations to be useful. The key technical contribution in this paper is an estimator we dub the `Dynkin estimator' that computes a treatment effect estimate directly under the steady-state distribution of the experimental policy. This estimator is biased but our main theoretical result establishes that this bias is small. Specifically, if the true treatment effect is $\delta$, then the bias of the Dynkin estimator is $O(\delta^2)$, wherein the suppressed constants depend {\em logarithmically} on the size of the state space. Our estimator relies on a relatively old idea in the RL literature, going back at least to \cite{kakadeApproximatelyOptimalApproximate2002}.
\newline
\textbf{2. Variance: }We show ({\bf Theorem \ref{th:dynkin_var}}) that the DQ estimator is asymptotically normal, and provide a non-trivial, explicit characterization of its variance. By comparison, we show ({\bf Theorem \ref{th:price}}) that this variance can, in general, be exponentially (in the size of the state space) smaller than the variance of {\em any} unbiased off-policy estimator. Our analysis introduces two new techniques. First, we prove what we dub an `Entrywise Non-expansive Lemma', that we believe is crucial to elucidating the variance reduction afforded by on-policy methods. Second, we introduce a novel linearization trick which dramatically simplifies the analysis of variance in RL via the delta method.  
%It is worth noting that the variance of off-policy estimators has not been characterized heretofore.

\noindent Summarizing the above points, we are the first (to our knowledge) to explicitly characterize the favorable bias-variance trade-off in using {\it on-policy} estimation to tackle off-policy evaluation. This new lens has broader implications for OPE and policy optimization in RL (e.g., this leads to a new approach with a provably lower bias than some widely used methods in policy optimization, see Section~\ref{sec:policy-optimization}).
%Combined with the previous point, the DQ estimator incurs a provably small bias for a massive reduction in variance.
%Implicit in the use of our estimator is the estimation of so-called $Q$-functions under a {\em fixed} policy. From an RL perspective, this is a relatively easy problem, and we are able to automatically leverage results going back to the thesis work of \cite{konda2002actor} that establish the asymptotic normality of several commonly-used estimators for this task.
\newline
\textbf{3. Practical Performance: }Despite the technical novelty described above, we view this as our most important contribution. We conduct experiments in both a caricatured one-dimensional environment proposed by others \cite{johari2022experimental}, as well as a city-scale simulator of a ride-sharing platform. We show that in both settings the DQ estimator has MSE that is substantially lower than (a) naive, and several state-of-the-art off-policy estimators, and even (b) estimators given access to incumbent state-of-the-art experimental {\em designs}.
%The remainder of this section will present a review of literature related to the Markovian interference problem and incumbent estimators. We also discuss important related tools from the Off-Policy evaluation and policy optimization literature.

\subsection{An Illustrative Example}
\label{sec:example}
It will be useful at this point to consider a simple example which highlights (a) the model of interference that we address, (b) the shortcomings of existing approaches to inference under such interference, and (c) our own approach to the problem.  {\em Importantly, all results presented in this simple example will extend to general MDPs by virtue of our analysis in Sections~\ref{sec:estimator} and \ref{sec:price}}.

Consider the continuous-time Markov chain depicted in \cref{fig:simple}; this is simply an $M/M/N/N$ queue (or the `Erlang B' model). The state space, ranging from 0 to $N$, can be thought of as the quantity of some resource (e.g.~rental homes of a similar type and geography) currently `occupied'. Customers arrive according to a Poisson process with rate $\lambda$, and independently with probability $p$, occupy a resource if available, for an exponentially-distributed duration with mean $1/\mu$. In spite of its simplicity, this model is closely related to one previously studied by  \cite{johari2022experimental} in the context of interference in commerce platforms.
\begin {figure}[!h]
\centering
\begin{tikzpicture}[->,line width =1pt, node distance =2.5cm]
	\node[circle, draw] (zero) [minimum size =14mm]{$0$};
	\node[circle, draw] (one) [right of=zero,minimum size =14mm] {$1$};
	\node[circle, draw] (two) [right of=one,minimum size =14mm]{$2$};
	\node[] (dot) [right of=two,minimum size =14mm]{...};
	\node[circle,draw] (N2) [right of=dot,minimum size =14mm]{$N-2$};
	\node[circle,draw] (N1) [right of=N2,minimum size =14mm]{$N-1$};
	\node[circle,draw] (N) [right of=N1,minimum size =14mm]{$N$};
	
	\path (zero) edge [bend left] node [above] {$p\lambda$} (one);
	\path (one) edge [bend left] node [above] {$p\lambda$} (two);
	\path (two) edge [bend left] node [above] {$p\lambda$} (dot);
	\path (dot) edge [bend left] node [above] {$p\lambda$} (N2);
	\path (N2) edge [bend left] node [above] {$p\lambda$} (N1);
	\path (N1) edge [bend left] node [above] {$p\lambda$} (N);
	
	\path (one) edge [bend left] node [below] {$\mu$} (zero);
	\path (two) edge [bend left] node [below] {$2 \mu$} (one);
	\path (dot) edge [bend left] node [below] {$3 \mu$} (two);
	\path (N2) edge [bend left] node [below] {$(N-2) \mu$} (dot);
	\path (N1) edge [bend left] node [below] {$(N-1) \mu$} (N2);
	\path (N) edge [bend left] node [below] {$N\mu$} (N1);
	
\end{tikzpicture}
\caption {A continuous-time Markov chain. Arrows indicate {\em rates} of transition between states.}
\label {fig:simple}
\end{figure}

Now consider a treatment whose effect is to increase the probability $p$ by some (unknown) quantity $\delta \ge 0$. Our goal is to measure the effect of the treatment on the steady-state rate of occupation (i.e. the steady-state rate of rightward transitions). We wish to estimate the treatment effect from a simple A/B test; i.e., an experiment that randomly applies (or does not apply) the treatment to each arriving customer. We now describe the various candidate estimators under this experimental design.

% \footnote{One precise instantiation of this randomization is the following: assume that the $\mathrm{Poisson}(\lambda)$ process, which we use to represent arriving customers who will occupy an available resource, is a sub-process of another Poisson process that represents {\em all} arriving customers, some of whom choose not to occupy a resource. The effect of the treatment is on this choice likelihood, and the randomization referred to here is exactly an A/B test: each arriving customer is either treated or not treated randomly.}

\paragraph{Existing Approach 1 -- Naive:} Given the observed trajectory during this experiment, the `naive' approach measures the empirical rates at which customers with and without treatment occupy resources, and takes the difference -- effectively ignoring interference. While this is largely what is done in practice, unfortunately the resulting estimator is {\em biased}. Specifically, its expected value overestimates the true treatment effect, loosely because it ignores the fact that an increase in $p$, while increasing the immediate likelihood of occupation, has the secondary effect of {\em decreasing} the availability of resources, and thus preventing new occupations in the future. This is {\em interference}.

\begin {figure}[!h]
\centering
\begin{tikzpicture}[->,line width =1pt, node distance =2.5cm]
	\node[circle, draw] (zero) [minimum size =10mm]{$0$};
	\node[circle, draw] (one) [right of=zero,minimum size =10mm] {$1$};
	
	\path (zero) edge [bend left] node [above] {$p\lambda$} (one);
	\path (zero) edge [loop left] node {$(1-p)\lambda + \mu$} (zero);
	\path (one) edge [bend left] node [below] {$\mu$} (zero);
	\path (one) edge [loop right] node {$\lambda$} (one);

%	\node[circle, draw] (zeroT) [minimum size =10mm] at (9,0) {$0$};
%	\node[circle, draw] (oneT) [right of=zeroT,minimum size =10mm] {$1$};
%	
%	\path (zeroT) edge [bend left] node [above] {$(p+\delta)\lambda$} (oneT);
%	\path (zeroT) edge [loop left] node {$(1-p-\delta)\lambda + \mu$} (zeroT);
%	\path (oneT) edge [bend left] node [below] {$\mu$} (zeroT);
%	\path (oneT) edge [loop right] node {$\lambda$} (oneT);
%
%	
\end{tikzpicture}
\caption {The discrete Markov chain analogous to the continuous-time chain depicted in \cref{fig:simple}, for the case $N=1$. %{\bf Left} is the control chain, and {\bf right} is the treatment chain. 
Arrows indicate transition {\em probabilities}, rather than rates. Without loss of generality, the parameters are normalized so that $\lambda + \mu = 1$.}
\label {fig:simple2}
\end{figure}

To be concrete, consider the simplest case: $N=1$. \cref{fig:simple2} depicts the equivalent {\em discrete} Markov chain, where we have assumed (without loss of generality) that $\lambda + \mu = 1$. A new occupation occurs whenever the chain transitions from state 0 to state 1. We are interested in the rate of such transitions, which can be worked out to be $p\lambda\mu/(p\lambda + \mu)$. The additive increase in this term when $p$ is replaced with $p + \delta$, is the so-called {\em average treatment effect} (ATE) that we are after. For this example, it suffices to know that the ATE is $\Omega(\delta)$.

The chain we actually observe, e.g.~resulting from an A/B test, applies the treatment with $1/2$ probability at each time period, affecting the transition probabilities when in state 0. Given a single trajectory $\{s_t\}$ of length $T$ from this chain, the {\em Naive} estimator then is
\[\hat{\rm ATE}_{\rm NV} =  \frac{1}{|T_1|} \sum_{t\in T_1} \I{s_{t}=0,s_{t+1}=1} - \frac{1}{|T_0|} \sum_{t\in T_0} \I{s_{t}=0,s_{t+1}=1},  \]
where $T_1$ and $T_0$ are, respectively, the sets of time periods in which the treatment was and was not applied. An explicit calculation then shows 
\begin{equation} \label{eq:simple} 	
\left\lvert 
\lim_T \hat{\rm ATE}_{\rm NV}  - {\rm ATE} 
\right\rvert 
\approx 
\frac{p\lambda}{\mu} {\rm ATE},
\end{equation} 
where the approximation ($\approx$) hides terms of size $O(\delta^2)$.
In words, unless the system is extremely unoccupied ($\mu \gg p\lambda$), the Naive estimator {\em has bias that is on the order of the treatment effect}. It is worth noting that the variance of this Naive estimator is effectively $O(1)$ -- i.e. it is as small as we can hope for. 

\paragraph{Existing Approach 2 -- Off-Policy Evaluation:}
We may view the problem at hand as one of {\em Off-Policy Evaluation} in reinforcement learning. To do this, we associate an MDP with our chain. The actions in this MDP correspond to treating or not treating an arrival at a given state in the chain. The reward associated with this action is 1 if the subsequent transition is to the right and 0 otherwise. The ATE then corresponds to the difference in average steady-state rewards between the two policies which always select, respectively, the treatment and non-treatment actions.

The task of estimating the ATE is now trivially viewed as one of OPE. This in turn, immediately suggests a whole host of existing OPE estimators that yield {\em unbiased} estimates of the ATE, e.g.~\cite{jiang2016doubly,kallus2020double,kallus2022efficiently}. This natural approach appears to be promising, e.g.~\cite{shi2020reinforcement}, but outside of secondary issues (e.g.~discounted vs.~average reward), the primary issue is that being unbiased appears to come at a price: variance. Specifically, one may show that {\em any} unbiased OPE estimator has variance that grows {\it exponentially} with the number of states in our chain, as $e^{\Omega(N)}$.

This sets up two extremes of a bias-variance tradeoff in our simple example: the Naive estimator has $O(1)$ variance, but its bias is on the order of the treatment effect itself. Any unbiased OPE estimator on the other hand will have variance that scales like $e^{\Omega(N)}$.

\paragraph{Our Approach -- The DQ Estimator:} Continuing to keep in mind the MDP policy evaluation lens from above, observe that the Naive estimator effectively computes the average difference in instantaneous rewards, averaged over states visited under the policy corresponding to simple randomization. Our estimator makes one change to the Naive estimator: instead of computing the average difference in instantaneous rewards, we instead compute the average difference in {\em Q-functions} \footnote{Q-functions are formally introduced in Section~\ref{sec:estimator}.}. Intuitively, doing so allows us to partially account for the long-term effects of selecting the treatment over no-treatment at any given state, and consequently, we hope for a less biased estimate of the treatment effect.

It turns out that the DQ estimator (denoted by $\hat{{\rm{ATE}}}_{\rm{DQ}}$) provides a dramatic reduction in bias. Starting with bias, the DQ estimator's bias can be worked out explicitly here, 
\begin{align*}
\left|\lim_{T} \hat{{\rm{ATE}}}_{\rm{DQ}} - {\rm{ATE}}\right| \approx \frac{\delta}{2} \frac{\lambda}{(\mu+\lambda p)} {\rm{ATE}}
\end{align*}
from which we find that it is $O(\delta^2)$. See Appendix \ref{sec:calculation-example} for details. This is second order relative to the ATE, and, of course, a marked improvement over the Naive estimator's bias. It turns out that this reduction in bias is generic: one of our primary contributions ({\bf Theorem \ref{th:dynkin_bias}}) is to prove the DQ estimator's bias is $O(\delta^2)$ in general MDPs.



Turning next to variance, we can show that the variance of the DQ estimator in our example is $O(N)$. In contrast, an optimal unbiased estimator has variance $e^{\Omega(N)}$, so that the DQ estimator provides an exponential reduction in variance for a relatively small increase in bias. In fact, these relative merits are also generic. Specifically, in {\bf Theorem \ref{th:dynkin_var}} we upper bound the variance of the DQ estimator for general MDPs. This upper bound scales as $\log(1/\rho_{\rm min})$, where $\rho_{\rm min}$ is probability of the least-visited state under the stationary distribution, which can be as large as $1/N$; in the given example $\rho_{\rm min} = e^{-\Omega(N)}$. In {\bf Theorem \ref{th:cramer-rao}} we prove a lower bound on the variance of {\em any} unbiased estimator in the context of general MDPs, which is exponentially larger -- scaling as $\Omega(1/\rho_{\rm min})$. These two bounds show that the variance reduction relative to OPE is generic ({\bf Theorem \ref{th:price}}).


% second of our primary contributions is to show formally that OPE estimators incur a price in variance that can be substantially higher than that of the DQ estimator. Specifically, we prove an upper bound ({\bf Theorem \ref{th:dynkin_var}}) on the variance of the DQ estimator, and a generic lower bound ({\bf Theorem \ref{th:cramer-rao}}) on the variance of {\em any} unbiased estimator. Combining these two results, we can upper bound the relative variance of the DQ estimator vs.~any OPE estimator, for any system. One consequence is that we can show constructively that there exist systems ({\bf Theorem \ref{th:price}}) for which OPE estimators have  {\em exponentially} larger (in the number of states) variance. But even outside of hand-constructed examples, we see the same effect in `real' systems, e.g.~\cref{fig:simple-plot} shows the relative variance in our running example for different values of $N$.


% \cref{fig:simple-plot} (Left) shows the relative bias of our DQ estimator vs.~the Naive estimator in the case $N=5000$, and the result is equally striking.
%One of our primary contributions ({\bf Theorem \ref{th:dynkin_bias}}) is to prove this in great generality: the DQ estimator's bias is {\em second-order} in the size of the treatment effect.



%Now without diving into the full notation and definitions (which will be introduced in Section \ref{sec:model}), one interpretation of our estimator is that it seeks to replace the instantaneous rewards in the Naive estimator with the experimental policy's $Q$-function -- this commonly-used quantity in reinforcement learning loosely measures the relative `advantage' of selecting a particular action at a particular state, assuming the given policy is applied at all times afterward. Thus, a difference in $Q$-function values should more precisely measure the long-term effect of an action, which is exactly what our {\em Differences-In-Q's (DQ)} estimator computes.

%Returning to our running example, the $Q$-function effectively shrinks the instantaneous reward by a factor of about $\mu/(p\lambda + \mu)$; comparing this term to the factor in \eqref{eq:simple} reveals that a reduction in bias occurs. In fact, the DQ estimator's bias can also be worked out explicitly, from which we find that it is $O(\delta^2)$, a marked improvement over the Naive estimator's $\Omega(\delta)$ bias. This reduction in bias is not unique to the $N=1$ case: \cref{fig:simple-plot} (Left) shows the relative bias of our DQ estimator vs.~the Naive estimator in the case $N=5000$, and the result is equally striking.
%One of our primary contributions ({\bf Theorem \ref{th:dynkin_bias}}) is to prove this in great generality: the DQ estimator's bias is {\em second-order} in the size of the treatment effect.

% \begin{figure}[h]
%  \centering
% \includegraphics[width=.9\textwidth]{../../fig/theory-bias-variance.pdf}
%  \caption{Comparison of estimators for a simple example from \cite{johari2022experimental}. {\it Left}: The relative bias of the DQ estimator over the Naive estimator, as a function of $\delta$, for $N=5000$. All biases are computed explicitly. We observe that this ratio is linear in $\delta$, as Theorem~\ref{th:dynkin_bias} predicts.
%  {\it Right}: The relative variance of the DQ estimator over any off-policy evaluation estimator (or  any  unbiased estimator), as a function of $N$. The DQ estimator's variance is approximated by its theoretical upper bound, and the off-policy estimator's variance is approximated by its theoretical lower bound. We can see that this ratio drops exponentially as $N$ increases, as in Theorem~\ref{th:dynkin_var} and \ref{th:cramer-rao}.}
%  \label{fig:simple-plot}
% \end{figure}

%The second of our primary contributions is to show formally that OPE estimators incur a price in variance that can be substantially higher than that of the DQ estimator. Specifically, we prove an upper bound ({\bf Theorem \ref{th:dynkin_var}}) on the variance of the DQ estimator, and a generic lower bound ({\bf Theorem \ref{th:cramer-rao}}) on the variance of {\em any} unbiased estimator. Combining these two results, we can upper bound the relative variance of the DQ estimator vs.~any OPE estimator, for any system. One consequence is that we can show constructively that there exist systems ({\bf Theorem \ref{th:price}}) for which OPE estimators have  {\em exponentially} larger (in the number of states) variance. But even outside of hand-constructed examples, we see the same effect in `real' systems, e.g.~\cref{fig:simple-plot} shows the relative variance in our running example for different values of $N$.

In summary, this example illustrates precisely the bias-variance trade-offs embodied by each estimator in Table~\ref{tab:bias-variance}. In particular, the DQ estimator has bias second-order in the estimand, with variance exponentially smaller than any unbiased OPE estimator --- capturing a particularly advantageous spot in the bias-variance curve. These results hold in generality for a large class of problems, which we formalize in the next section.

\begin{table}[h!]
\centering
\begin{tabular}{@{}lcc@{}} \toprule
	{\bf Estimator} & {\bf Bias} & {\bf Variance} \\ \midrule
	Naive & $\Omega(\delta)$ & $O(1)$  \\
	Off-Policy Evaluation & 0 & $e^{\Omega(N)}$ \\
	Differences-In-Q's (DQ) & $O(\delta^2)$ & $O(N)$ \\ \bottomrule
\end{tabular}
\caption{The bias-variance tradeoff of different estimators. Bias is parameterized by the additive impact $\delta$ of the intervention on transition probabilities -- note that the ATE itself can be $\Omega(\delta)$. `Variance' shows the limiting variance of each estimator on this example, as a function of the cardinality $N$ of the state space. In full generality, variance is $O(\log (1 / \rho_{\rm \min}))$ for DQ, and $\Omega(1/\rho_{\min})$ for OPE, where $\rho_{\rm min}$ is the frequency of the least-visited state under the steady-state distribution. In this example $\rho_{\rm min} = e^{-\Omega(N)}$, but in general $\rho_{\rm min}$ can be up to $1/N$.}
\label{tab:bias-variance}
\end{table}

\paragraph{Aside -- Alternative Experimental Designs: }

Whereas our focus is on estimation assuming simple-randomization, a more sophisticated {\it two-sided randomization} (TSR) design has also been studied for this specific system in \cite{johari2022experimental}. In their scheme, both customers {\it and} resources are randomized independently into treatment and control, and the intervention is applied only if both the customer and the resource are treated. We provide empirical comparisons against this approach in Section~\ref{sec:experiments}, which show that DQ outperforms TSR in typical supply / demand regimes, despite a simpler design. 

% Finally, we note that more sophisticated experimental designs can be applied here -- (\cite{johari2022experimental}) %



%\vspace{-1em}
% \paragraph{Our Contributions:}
% Zooming out from our example, we can now describe our contributions precisely.
% We study a generic experimentation problem within a system represented as a Markov Decision Process (MDP), where treatment corresponds to an action which may interfere with state transitions. This form of interference, which we refer to as {\em Markovian}, naturally subsumes the platform examples alluded to earlier, as recently noted by others either implicitly \cite{qinReinforcementLearningRidesharing2021} or explicitly \cite{johari2022experimental,shi2020reinforcement}. In that example, a user arrives at each time step, the platform chooses an action (whether to treat the user), and the user's purchase decision alters the system state (inventory levels).
% Our goal is to estimate the Average Treatment Effect (ATE), defined as the difference in steady-state reward with and without applying the treatment. In light of the above discussion, we assume that experimentation is done under simple randomization (i.e.~A/B testing).
%%Now without design as a lever, there are perhaps two existing families of estimators:
%%\newline
%%\textbf{1. Naive:} We will explicitly define the {\em Naive} estimator in the next section, but the strategy amounts to simply ignoring the presence of interference. This is by and large what is done in practice. Of course it may suffer from high bias (we show this formally in Example \ref{eg:two_state}), but it serves as more than just a strawman. In particular, bias is only one side of the estimation coin, and with respect to the other side, namely variance, the Naive estimator is effectively the best possible.
%%\newline
%%\textbf{2. Off-Policy Evaluation (OPE):} Another approach comes from viewing our problem as one of policy evaluation in reinforcement learning (RL). Succinctly, it can be viewed as estimating the average reward of two different policies (no treatment, or treatment) given observations from some {\em third} policy (simple randomization). This immediately suggests framing the problem as one of {\em Off-Policy Evaluation}, and borrowing one of many existing {\em unbiased} estimators, e.g.~\cite{thomas2015high,thomas2016data,liu2018breaking,jiang2016doubly,kallus2020double,kallus2022efficiently}. This tack appears to be promising, e.g.~$\cite{shi2020reinforcement}$, but we observe that the resulting variance is necessarily large (Theorem \ref{th:cramer-rao}).
%
%%State-of the-art estimators for this problem proposed in recent years attempt to heuristically correct for the interference between experimental units and thus mitigate bias. But the extent to which these estimators mitigate the problem at hand is largely only understood experimentally. The problem at hand is a hard one since real-world experiments with such interference often have limited experimentation budgets, which ends up ruling out more sophisticated estimators due to their variance. 
%
%%\vspace{-1em}
%\paragraph{Our Contributions:}

\subsection{Related Literature:}

%The notion of interference in experiments can be formally traced back to at least \cite{struchiner1990behaviour,talbot1995effect,lucking-reileyUsingFieldExperiments1999} in the contexts of public medicine, farming, and online markets, respectively, and has re-appeared in multiple modern contexts including, e.g., social networks \cite{aral2011creating}, ride-sharing \cite{lyft2022experimentation}, and lodging rentals \cite{johari2022experimental}. Many of these applications fall under our notion of `Markovian' interference, whether implicitly or explicitly (e.g. \cite{qinReinforcementLearningRidesharing2021} for ride-sharing).


The largest portion of work in interference is in {\em experimental design}, with the design levers ranging from stopping times in A/B tests \cite{kharitonov2015sequential,johari2017peeking,yang2017framework,JohPekWal2020Always}, to any form of more-sophisticated `clustering' of units \cite{cornfield1978symposium,farquhar1978symposium,commit1991community,donner2004pitfalls,murray1998design,ugander2013balanced,walker2014design,eckles2017design,farias2021learning}, to clustering specifically when interference is represented by a network \cite{manski2013identification,ugander2013graph,saveski2017detecting,athey2018exact,basse2019randomization,pouget2019variance,zigler2021bipartite}, to the proportion of units treated \cite{hudgens2008toward,tchetgen2012causal,baird2018optimal}, to the timing of treatment \cite{sneider2018experiment,bojinov2020design,glynnAdaptiveExperimentalDesign2020}, and beyond \cite{backstrom2011network,katzir2012framework,toulis2013estimation,manski2013identification,choi2017estimation,basse2018model,gui2015network,saveski2017detecting,farias2022synthetically}. As alluded to earlier, these sophisticated designs can be powerful, but cost, user experience, and other implementation concerns restrict their application in practice \cite{kirnChallengesExperimentation2022,kohavi2020trustworthy}.

We view this paper as orthogonal to this literature, but will eventually compare against a recent state-of-the-art design, so-called {\em two-sided randomization} \cite{johari2022experimental,bajari2021multiple}, that is specific to the context of two-sided marketplaces (e.g.~the one we simulate).

%, which mitigates bias for `naive' estimators via sophisticated experimental design. Instead, for reasons including cost and organizational friction, experimentation on online platforms in particular still largely relies on the simplest designs (customer randomization in particular). Our contribution is a (slightly) more sophisticated estimator that applies to a simple set of designs, which includes customer randomization, and can be extended easily to the recently-developed `two-sided' randomization appraoch \cite{johari2022experimental,li2021interference,bajari2021multiple} (a hybrid in the above taxonomy), as we discuss in Section \ref{sec:alternatives}.

%
%Marketplace-specific:
%\begin{itemize}
%\item \cite{blake2014marketplace}: Early instance of marketplace interference concerns.
%\item \cite{wager2021experimenting}: Another model for interference in marketplace settings.
%\item \cite{holtzLimitingBiasTestControl2020}: Network interference model of interference in marketplaces.
%\end{itemize}



%\paragraph{Mitigating Interference via Experimental Design:}



%Switchback: \cite{sneider2018experiment,bojinov2020design}. \cite{glynnAdaptiveExperimentalDesign2020}: Adaptive design of switchbacks in a Markov chain model (with Markov chain interference).

%Two-sided experimentation
%\begin{itemize}
%\item \cite{johari2022experimental}:  Hannah Li's paper.
%  \item \cite{li2021interference}: The follow-up of the previous one that considers a static setting.
%\item \cite{bajari2021multiple}: Generalizations of two-sided randomization for marketplace settings.
%\end{itemize}

%\textbf{Estimation via Reinforcement Learning:}
As stated earlier, the problem we study is one of {\em off-policy evaluation (OPE) }\cite{precup2001off,sutton2008convergent}. %, itself a classic problem in reinforcement learning.
The fundamental challenge in OPE %, which we view as one reason why we cannot simply port one of the many existing unbiased estimators to our problem,
is high variance, which can be attributed to the nature of the algorithmic tools used, e.g. sampling procedures \cite{thomas2015high,thomas2016data,liu2018breaking}. Recent work on `doubly-robust' estimators \cite{jiang2016doubly,kallus2020double,kallus2022efficiently} has improved on variance (incidentally, our estimator is loosely tied to these, as we discuss in Section \ref{sec:conclusion}), but again we will show, via a formal lower bound, that unbiased estimators as a whole have prohibitively large variance. Finally, our motivation is close in spirit to a recent paper \cite{shi2020reinforcement}, which applies OPE directly in Markovian interference settings; we make a direct experimental comparison in Section \ref{sec:experiments}.

In the policy optimization literature, `trust-region' methods \cite{schulman2015trust} and conservative policy iteration \cite{kakadeApproximatelyOptimalApproximate2002} use a related on-policy estimation approach to bound policy improvement. Relative to the existing literature, we develop an on-policy surrogate with provably lower bias than extant proposals; see Section~\ref{sec:policy-optimization}. Furthermore, the explicit application of on-policy estimation in the context of OPE, and in particular the striking bias-variance tradeoff this enables, are novel to this paper.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> Tex Files/Model.tex <==
\section{Model} \label{sec:model}
Having discussed each estimator in a specific example, we now formalize the general inference problem that we tackle, casting it in the language of MDPs. Vis-\`{a}-vis the existing literature, this lens allows us to reason about the problem using a large, well-established toolkit, and makes obvious the fact that OPE provides unbiased estimation of the ATE. We then present what we call the `Naive' estimator (alluded to in the introduction). This is the lowest-variance estimator one can hope for in this setting, but it can have significant bias, as we see in \cref{eq:simple}.

% We then briefly discuss two state-of-the-art alternatives to the Naive estimator: the TSR estimator \cite{johari2022experimental} that supposedly mitigates bias while also being low variance, and Off-Policy evaluation (which, thanks to our problem framing is an obvious unbiased alternative). Finally, we present our proposal -- the DQ estimator.

We begin by defining an MDP with state space $\Sscr$. We denote by $s_t \in \Sscr$ the state of the MDP at time $t \in \mathbb{N}$. Every state is associated with a set of available actions $\Ascr$ which govern the transition probabilities between states via the (unknown) function $p:\Sscr \times \Ascr \times \Sscr \to [0,1]$. We assume that $\Ascr = \{0,1\}$ irrespective of state; for descriptive purposes, we will associate the `$1$' action with the use of a prospective intervention, so that `$0$' is associated with not employing the intervention. We denote by $r(s,a)$ the reward earned in state $s$ having employed action $a$. A policy $\pi: \Sscr \rightarrow \Ascr$ maps states to random actions. We define the average reward $\lambda^\pi$, under any (ergodic, unichain) policy $\pi$, according to:
\[
\lambda^\pi = \lim_{T \to \infty} \frac{1}{T} \sum_{t=1}^T r(s_t,\pi(s_t)).
\]
There are three policies we define explicitly: 

\textbf{The Incumbent Policy $\pi_0$: }This policy never uses the intervention, so that $\pi_0(s) = 0$ for all $s$. This is `business as usual'. Denote the associated transition matrix as $P_{0}$ (i.e. the entries of $P_0$ are exactly $p(\cdot,0,\cdot)$)

\textbf{The Intervention Policy $\pi_1$: }This policy always uses the intervention, so that $\pi_1(s) = 1$ for all $s$. This reflects the system, should the intervention under consideration be `rolled out'. Denote the associated transition matrix as $P_{1}$.

\textbf{The Experimentation Policy $\pi_{p}$: }This policy corresponds to the experiment design. Simple randomization would select $\pi(s) = 1$ with some fixed probability $p$, say $1/2$, independently at every period. This corresponds to the sort of search engine experiment alluded to in the introduction. The transition matrix associated with this design is then $P_{1/2} = \frac{1}{2}P_{0} + \frac{1}{2}P_{1}$.

% Relative to the sort of search engine experiment alluded to in the introduction, the state of the above MDP might codify the available inventory of various products on the platform, with each time step corresponding to a user search, and transitions in the state driven by potential purchases. A much more careful modeling exercise is presented in Section~\ref{sec:experiments} in the context of ride-hailing. We are now in a position to state the inference problem we will tackle:
%
\noindent\textbf{\textsf{The Inference Problem: }}We are given a single sequence of $T$ states, actions, and rewards, observed under the experimentation policy $\pi_p$ (recall that cost and constraints \cite{kirnChallengesExperimentation2022,kohavi2020trustworthy} prohibit us from running $\pi_{0}$ or $\pi_{1}$ separately until convergence). We observe the sequence  $\{(s_t, a_t, r(s_t,a_t)): t = 1,\dots,T\}$, wherein $a_t \triangleq \pi_p(s_t)$. Our goal is to estimate the average treatment effect (ATE): ${\rm ATE} \triangleq \lambda^{\pi_1} - \lambda^{\pi_0}. $

\noindent\textbf{\textsf{The Naive Estimator and Bias.}} A natural approach to estimating the ATE is to use simple randomization (i.e.~$P_{1/2}$) and  the {\em Naive} estimator, which we define in the language of MDPs as: $\hat{\rm ATE}_{\rm NV} =  \frac{1}{|T_1|} \sum_{t\in T_1} r(s_t,a_t) - \frac{1}{|T_0|} \sum_{t\in T_0} r(s_t,a_t),$
where $T_1 = \{t: a_t =1\}$ and $T_0 = \{t: a_t =0\}$. In the context of the example of Section~\ref{sec:example}, this corresponds to simply taking the difference between the probability of renting a resource among test users ($T_1$), and control users ($T_0$). What goes wrong is simply that the two empirical averages above, that seek to estimate $\lambda^{\pi_1}$ and $\lambda^{\pi_0}$ respectively, employ the wrong measure over states.
%In particular, $\lambda^{\pi_1}$ ought to be calculated under the stationary distribution induced by $\pi_1$, and $\lambda^{\pi_0}$ ought to be calculated under the stationary distribution induced by $\pi_0$, but the estimator above attempts to calculate both these averages under the stationary distribution induced by the policy $\pi_p$.
As we saw, this is sufficient to introduce bias that is on the order of the treatment effect being estimated.
% \begin{example}
% \label{eg:two_state}
% Consider an MDP on two states, $\Sscr = \{\mathbf{0},\mathbf{1}\}$. We collect a reward of $0$ in state $\mathbf{0}$ irrespective of the  action taken in that state $(r(\mathbf{0}, 0)=r(\mathbf{0},1)=0)$, and a reward of $1$ in state $\mathbf{1}$, again, irrespective of action $(r(\mathbf{1},0) = r(\mathbf{1},1)=1)$. On the other hand, transitions are impacted by our choice of action. Specifically, let $p(\mathbf{0},0,\mathbf{0}) = p(\mathbf{0},0,\mathbf{1}) = p(\mathbf{1},0,\mathbf{1}) = p(\mathbf{1},0,\mathbf{0}) = 1/2$. We maintain
% $p(\mathbf{0},1,\mathbf{1}) = p(\mathbf{0},1,\mathbf{0}) = 1/2$ so that the intervention has no effect at state $\mathbf{0}$. On the other hand, we let  $p(\mathbf{1},1,\mathbf{1}) = 1/2 + \delta$, so that $p(\mathbf{1},1,\mathbf{0}) = 1/2 - \delta$, for some $\delta > 0$. In words, the intervention tends to discourage a transition to $\mathbf{0}$ from state $\mathbf{1}$.
% \end{example}
% \addtocounter{example}{-1}

% In the above example, it is easy to calculate that ${\rm ATE} = ({1}/{2}) {\delta}/({1-\delta})$, reflecting the shift in the stationary distribution favoring state $\mathbf{1}$, induced under the intervention. On the other hand, we can calculate that $\lim_T \hat{\rm ATE}_{N} = 0$, so that the bias induced by the `experimentation' policy relative to the stationary distributions under the incumbent and intervention policies respectively, is comparable to the size of the treatment effect.

%\subsection{Alternatives} \label{sec:alternatives}
%
%Our formulation is a special case of Off-policy evaluation, and as such that entire body of unbiased estimators can be brought to bear on the present problem. We address these estimators more carefully in Sections~\ref{sec:connection} and \ref{sec:price}, but for now simply note that while unbiased, these estimators naturally have (much) higher variance than the Naive estimator~\eqref{eq:naive} which limits their use in the presence of limited experimentation budgets (i.e. small $T$). 
%
%Can we mitigate bias while maintaining variance at the level of Naive estimation with simple randomization? \cite{johari2022experimental} and \cite{bajari2021multiple} recently proposed `Two-sided' randomization as one potential approach. The approach applies a distinct experimental design that is only applicable to a certain class of MDPs; we implement this approach in our computational experiments and describe the details of the approach further in Appendix A. 
%




%How do we fix this bias? One approach is the following: continuing with Example~\ref{eg:two_state}, imagine we attempted to estimate the transition probabilities $p(s,a,s')$ for every $(s,a,s')$; in the context of the example, this is a set of $8$ probabilities. Given these, we could compute asymptotically (in $T$) unbiased estimates of $\lambda^{\pi_1}$ and $\lambda^{\pi_0}$, thereby yielding an asymptotically unbiased estimate of the ATE. This is the essence of the off-policy estimation approach to the problem at hand, as exemplified by~\cite{.}. It is not hard to imagine that any estimator constructed in this fashion is likely to have high variance, and this is indeed what one observes in practice (as we will in Section~\ref{}). 

%\subsection{Real World Applications}
%
%What fits/ what doesn't. Point to section on extensions to deal with two-sided randomization. [AALI]
%
%Evaluating the effects of
%different order dispatching strategies in ride-sharing companies (e.g., Uber) for large-scale
%fleet management \cite{shi2020reinforcement}

%\cite{wager2021experimenting}: examples with continuous treatment arm, e.g. renewable energy subsidies
%
%Congestion pricing \cite{goh2002congestion}







%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> Tex Files/Proof-main.tex <==
%
%\section{Proof of Theorem \ref{th:dynkin_bias}}
%%The proof is a simple proof based on observing a particular way of parameterizing ATE as a function of $\delta$. Turns out the Taylor expansion of such a function reveals naturally the bias-correction results of corresponding estimators (Naive estimator is the zeroth-order Taylor expansion, the DQ estimator is the first-order Taylor expansion, et.al). 
%%
%%Before getting started, let us denote a few vectors for notational convenience. Let $\rho_{0} \in \R^{|\Sscr|}, \rho_{1/2} \in \R^{|\Sscr|}, \rho_{1} \in \R^{|\Sscr|}$ be the vectors of the stationary distributions of $P_0, P_{1/2}, P_{1}$ accordingly. Let $r_0 \in \R^{|\Sscr|}, r_{1/2} \in \R^{|\Sscr|}, r_1 \in \R^{|\Sscr|}$ be the reward vectors associated with policies $\pi_0, \pi_{1/2}, \pi_{1}$, i.e., $r_{a}(s) = r(s, a)$ and $r_{1/2} = \frac{1}{2} r_0 + \frac{1}{2} r_1.$
%%
%%To begin, we parameterize $P_0 := P_{1/2} - \delta A$ and $P_1 := P_{1/2} + \delta A$ by $\delta$ with fixed $P_{1/2}$ and some fixed matrix $A \in \R^{|\Sscr|\times |\Sscr|}$ with $\|A\|_{1,\infty} \leq 1.$ Therefore, $\rho_{0}$ and $\rho_{1}$ can also be viewed as a function of $\delta.$ Also recall ${\rm{ATE}} = \rho_{1}^{\top} r_{1} - \rho_{0}^{\top} r_0$. Our goal is to represent ${\rm{ATE}}$ as a function of $\delta$ and then study the Taylor expansion of such a function. 
%%
%%To do so, let us state the following known perturbation formula of Markov chains. 
%%\begin{lemma}[Stationary Distribution Perturbation, Theorem 4.1 \cite{meyer1980condition}]\label{lem:perturbation-stationary-distribution}
%%Suppose $P \in \R^{n \times n}$ and $P' \in \R^{n\times n}$ are transitions matrices of two finite-state aperiodic and irreducible Markov Chains and $\rho \in \R^{n}, \rho' \in \R^{n}$ are the stationary distributions accordingly. Then
%%\begin{align*}
%%\rho'^{\top} = \rho^{\top} + \rho'^{\top} (P' - P) (I - P)^{\#}
%%\end{align*} 
%%where $(I-P)^{\#}$ is the group inverse of $I-P$ given by $(I-P)^{\#}=(I-P+\one \rho^{\top})^{-1} - \one \rho^{\top}.$
%%\end{lemma}
%%Let us apply \cref{lem:perturbation-stationary-distribution} to $\rho_{1}^{\top} r_1$ based on the perturbation between $\rho_{1/2}$ and $\rho_{1}$.
%%\begin{align}
%%\rho_1^{\top} r_1 
%%&= \rho_{1/2}^{\top} r_1 + \rho_{1}^{\top} (P_1 - P_{1/2}) (I-P_{1/2})^{\#} r_1 \nonumber\\
%%&= \rho_{1/2}^{\top} r_1 + \delta \cdot \rho_{1}^{\top} A (I-P_{1/2})^{\#} r_1 \label{eq:expansion-rho-rho1}
%%\end{align}
%%Note that we can apply \cref{lem:perturbation-stationary-distribution} again to the $\rho_{1}$ in the RHS of \cref{eq:expansion-rho-rho1} and obtain
%%\begin{align}
%%\rho_1^{\top} r_1 
%%&= \rho_{1/2}^{\top} r_1 + \delta \cdot \rho_{1/2}^{\top} A (I-P_{1/2})^{\#} r_1 + \delta^2 \cdot \rho_{1}^{\top} \left(A (I-P_{1/2})^{\#}\right)^2 r_1 \label{eq:expansion-rho-rho1-second}
%%\end{align}
%%Repeat this process, then for any $K = 0, 1, 2, \dotsc$, we have
%%\begin{align}
%%\rho_1^{\top} r_1 
%%&= \sum_{k=0}^{K} \delta^{k} \cdot \rho_{1/2}^{\top} \left(A (I-P_{1/2})^{\#}\right)^k r_1 + \delta^{K+1} \cdot \rho_{1}^{\top} \left(A (I-P_{1/2})^{\#}\right)^{K+1} r_1 \label{eq:expansion-rho-rho1-K}
%%\end{align}
%%Essentially \cref{eq:expansion-rho-rho1-K} provides the $K$-th order Taylor expansion for $\rho_{1}^{\top}r_1$ with an explicit remainder. Furthermore, we can bound the remainder by
%%\begin{align*}
%%\left|\rho_{1}^{\top} \left(A (I-P_{1/2})^{\#}\right)^{K+1} r_1\right| 
%%&\overset{(i)}{\leq} \norm{\rho_{1}}_{1} \left(\norm{A}_{1,\infty} \norm{I-P_{1/2}^{\#}}_{1,\infty}\right)^{K+1} \norm{r_1}_{\max}\\
%%&\overset{(ii)}{\leq} \norm{I-P_{1/2}^{\#}}_{1,\infty}^{K+1} r_{\max} \\
%%&\overset{(iii)}{\leq} \left(\frac{2\ln(C)+1}{1-\lambda}\right)^{K+1} r_{\max}
%%\end{align*}
%%Here in (i) we use that for any vector $a, b$ and matrix $B$, we have $|a^{\top}b| \leq \|a\|_{1}\|b\|_{\max}$ and $\norm{a^{\top}B}_{1} \leq \norm{a}_{1} \norm{B}_{1,\infty}$ with $\|\cdot\|_{1}$ being the $l_1$-norm and $\|B\|_{1,\infty} = \max_{i} \sum_{j} |B_{ij}|$ being the maximum absolute row sum norm. In (ii) we use that $\norm{\rho_1}_1 = 1, \norm{A}_{1,\infty} \leq 1$. In (iii), we use the fact that $\norm{(I-P_{1/2})^{\#}}_{1,\infty} \leq \frac{2\ln(C)+1}{1-\lambda}$ by the mixing time assumption (the proof is postponed to the end of this section).
%%
%%Similar process can be applied to $\rho_{0}^{\top}r_0$ and then we obtain the $K$-th order Taylor expansion for ATE.
%%\begin{align}
%%{\rm{ATE}} 
%%&= \rho_1^{\top} r_1 - \rho_0^{\top} r_0 \nonumber\\
%%&=  \sum_{k=0}^{K} \delta^{k} \cdot \left(\rho_{1/2}^{\top} \left(A (I-P_{1/2})^{\#}\right)^k r_1 - \rho_{1/2}^{\top} \left((-A) (I-P_{1/2})^{\#}\right)^k r_0\right) \nonumber\\
%%&\quad + \delta^{K+1} \cdot a_{K} \label{eq:taylor-expansion-ATE}
%%\end{align}
%%where $|a_{K}| \leq 2\left(\frac{2\ln(C)+1}{1-\lambda}\right)^{K+1} r_{\max}.$
%%
%%It is easy to see that the Naive estimator $\rho_{1/2}^{\top}(r_1-r_0)$ corresponds to the zeroth-order Taylor expansion. In fact, the DQ estimator, i.e., $\E_{\rho_{1/2}} \left[\tauDK \right]$, exactly matches the first-order expansion. To see this, by the definition of $\E_{\rho_{1/2}} \left[\tauDK \right]$ and $Q$-functions, 
%%\begin{align*}
%%\E_{\rho_{1/2}} \left[\tauDK \right] 
%%&= \sum_s \rho_{1/2}(s) \left(Q_{\pi_{1/2}}(s,1) - Q_{\pi_{1/2}}(s,0) \right) \\
%%&= \sum_{s} \rho_{1/2}(s) \left(r_1(s) +\sum_{s'} V_{1/2}(s')P_{1}(s,s') - r_0(s) - \sum_{s'} V_{1/2}(s')P_{0}(s,s')\right)\\
%%&= \rho_{1/2}^{\top} \left(r_1 - r_0 + (P_1-P_0)V_{1/2}\right)
%%\end{align*}
%%where $V_{1/2}$ is the induced vector of the $V$-function of policy $\pi_{1/2}.$ By the well-known fact that $V_{1/2} = (I-P_{1/2})^{\#} r_{1/2}$ induced by the Bellman equation, we then have
%%\begin{align*}
%%\E_{\rho_{1/2}} \left[\tauDK \right] 
%%&=  \rho_{1/2}^{\top} \left(r_1 - r_0 + (P_1-P_0)(I-P_{1/2})^{\#} r_{1/2}\right)\\
%%&= \rho_{1/2}^{\top} r_1  - \rho_{1/2}^{\top} r_0 + \delta A (I-P_{1/2})^{\#} (r_{1}+r_{0}).
%%\end{align*}
%%Then indeed $\E_{\rho_{1/2}} \left[\tauDK \right]$ is the first-order Taylor expansion in \cref{eq:taylor-expansion-ATE}. Together, this completes the proof:
%%\begin{align*}
%%\left|{\rm{ATE}} - \E_{\rho_{1/2}} \left[\tauDK \right]\right| \leq 2\delta^2 r_{\max}\left(\frac{2\ln(C)+1}{1-\lambda}\right)^2.
%%\end{align*}
%%\textbf{Generalization to Higher-Order Bias Correction.} In fact, the K-th order Taylor expansion of ATE allows us to design estimators that can correct higher-order bias, based on computing difference-in-Q functions iteratively. See details in \cref{sec:korder-correction}.
%%
%
%
%The only thing remaining is to bound $\norm{I-P_{1/2}}^{\#}$, for which we state in the following lemma. 
%\begin{lemma}\label{lem:group-inverse-L1}
%    Suppose $P \in \R^{|\Sscr|\times |\Sscr|}$ is the transition matrix of a finite-state aperiodic and irreducible Markov Chain and $\rho$ is the stationary distribution. Suppose there exists $C$ and $\lambda$ such that for any $k$ and $s \in \Sscr$, $d_{\rm TV} (P_{1/2}^{k}(s, \cdot), \rho_{1/2}) \leq C \lambda^{k}$,
%    Then
%    \begin{align*}
%        \norm{(I-P)^{\#}}_{1,\infty} \leq \frac{2\ln(C)+1}{1-\lambda}.
%    \end{align*}
%\end{lemma}
%\begin{proof}
%It is known that $(I-P)^{\#} = \sum_{k=0}^{\infty} \left( P^{k} - \one\rho^{\top}\right)$ by the series expansion of $(I-P)^{\#} := (I-P+\one\rho^{\top})^{-1} - \one\rho^{\top}$ and $(P-\one\rho^{\top})^{k} = P^{k} - \one\rho^{\top}$ for $k\geq 1.$ Then
%\begin{align*}
%    \norm{(I-P)^{\#}}_{1,\infty} 
%    &\leq \sum_{k=0}^{\infty} \norm{P^{k} - \one\rho^{\top}}_{1,\infty}\\
%    &\overset{(i)}{\leq} \sum_{k=0}^{\infty} \min\left(2, C \lambda^{k}\right)\\
%    &\leq \sum_{k=0}^{\log_{\lambda}(1/C)-1} 2 + \sum_{k=\log_{\lambda}(1/C)}^{\infty} C\lambda^{k}\\
%    &\leq 2\log_{\lambda}(1/C) + \frac{1}{1-\lambda}\\
%    &= 2\frac{\ln(C)}{-\ln(\lambda)} + \frac{1}{1-\lambda}\\
%    &\overset{(ii)}{\leq} \frac{2\ln(C)+1}{1-\lambda}
%\end{align*}
%where (i) is due to $\norm{P^{k}}_{1,\infty}, \norm{\one \rho^{\top}}_{1,\infty} \leq 1$ and $d_{\rm TV} (P_{1/2}^{k}(s, \cdot), \rho_{1/2}) \leq C \lambda^{k}$ and (ii) is due to $-\ln(x) \leq 1 - x$ for $x>0.$
%\end{proof}
%
%
%

%
%\section{Proof of Theorem \ref{th:dynkin_var}}\label{sec:proof-variance-bound}
%
%\subsection{Entry-wise Non-Expansive Lemma}
%To begin, we present a lemma that is the key enabler of establishing the striking variance improvement of the DQ estimator  over the un-biased estimator. The lemma simply states
%\begin{lemma}[Entry-wise non-expansive lemma]\label{lem:non-expansive-lemma}
%Let $W: \R^{|\Sscr|} \rightarrow \R^{|\Sscr|}$ be a map denoted by $W(\rho) := (I-P_{1/2})^{\#\top}(P_1-P_0)^{\top} \rho.$ Then, for any $s \in \Sscr$, 
%\begin{align*}
%\frac{1}{c}\left|W(\rho_{1/2}) (s)\right| \leq \rho_{1/2}(s)
%\end{align*}
%where $c := 4\frac{\ln(C) +  \ln \left(1/\rho_{\min}\right) + 1}{1-\lambda}.$
%\end{lemma}
%This is to say, the mapping $\frac{1}{c} W$ does not expand $\rho_{1/2}$ in terms of entry-wise values. To see the necessity of this lemma and gain some intuition, consider a special case where $P_{0}, P_{1}, P_{1/2}, \rho_0, \rho_1, \rho_{1/2}$ are all known, while only the rewards are unknown and can only be sampled under the distribution $\rho_{1/2}.$ For simplicity, assume $r_0=r_1=r$ and the sample for $r_{t} = r(s_t) + \epsilon_{t}$ is i.i.d from $\rho_{1/2}$ with some exogenous noise $\epsilon_{t} \sim \mathcal{N}(0, 1).$ Let us denote the empirical average estimator for $r$ be $\hat{r}.$ 
%By CLT, we have 
%$$
%\sqrt{T}(\hat{r}-r) \overset{d}{\rightarrow} \mathcal{N}(0, D^{-1})
%$$
%where $D$ is a diagonal matrix with entries $D_{s,s} = \rho_{1/2}(s).$ This limiting variance captures the intuition that, for the state that is rarely visited, the variance for $\hat{r}(s) - r(s)$ can blow up. In fact, consider an un-biased estimator $(\rho_{1}^{\top}-\rho_{0}^{\top})\hat{r}$ for the ATE, $(\rho_1^{\top}-\rho_0^{\top})r$, (this is the un-biased estimator that achieves the optimal variance), we have
%\begin{align*}
%\sqrt{T} \left((\rho_{1}^{\top}-\rho_{0}^{\top})\hat{r} - {\rm{ATE}}\right)\overset{d}{\rightarrow} \mathcal{N}(0, \sigma_{0}^2)
%\end{align*}
%where
%\begin{align*}
%\sigma_0^2 
%&:= (\rho_{1}^{\top}-\rho_{0}^{\top}) D^{-1} (\rho_{1}-\rho_{0})\\
%&= \sum_{s} \frac{(\rho_1(s) - \rho_0(s))^2}{\rho_{1/2}(s)}.
%\end{align*}
%Note that there is no guarantee for the likelihood ratio $\frac{\rho_0(s)}{\rho(s)}$ and $\frac{\rho_1(s)}{\rho(s)}$ and in general $\sigma_0^2 = \Omega\left(\frac{1}{\rho_{\min}}\right)$ and this is the price to pay for the un-biased off-policy evaluation. 
%
%On the other hand, one can verify that the DQ estimator is simply
%\begin{align*}
%{\rm{ATE}}_{D} = \rho_{1/2}^{\top} \left(P_0-P_1\right) (I-P_{1/2})^{\#} \hat{r}.
%\end{align*}
%This leads to the limiting variance of ${\rm{ATE}}_{\rm DQ}$:
%\begin{align*}
%\sqrt{T}\left({\rm{ATE}}_{D} - \E_{\rho_{1/2}}[{\rm{ATE}}_{D}]\right) \overset{d}{\rightarrow} \mathcal{N}(0, \sigma_{1}^2)
%\end{align*} 
%where 
%\begin{align*}
%\sigma_{1}^2 &:= \rho_{1/2}^{\top} \left(P_0-P_1\right) (I-P_{1/2})^{\#} D^{-1} (\rho_{1/2}^{\top} \left(P_0-P_1\right) (I-P_{1/2})^{\#})^{\top} \\
%&=  \norm{\rho_{1/2}^{\top} \left(P_0-P_1\right) (I-P_{1/2})^{\#} D^{-1/2}}^2.
%\end{align*}
%By the definition of $W$ mapping, we then have
%\begin{align*}
%\sigma_{1}^2 
%&= \sum_{s} \left(W(\rho_{1/2})(s) \frac{1}{\rho_{1/2}(s)^{1/2}}\right)^2\\
%&\overset{(i)}{\leq} \sum_{s} \frac{1}{c^2} \rho_{1/2}(s)\\
%&=  \frac{1}{c^2}.
%\end{align*}
%where (i) is due to \cref{lem:non-expansive-lemma}. Then $\sigma_{1}$ is in the order of $\log(1/\rho_{\min})$. In fact, without \cref{lem:non-expansive-lemma}, a loose analysis will provide $\sigma_{1}^2 = \Omega(1/\rho_{\min})$, which is in the same order of $\sigma_0^2$, that shows no advantage of using DQ estimator. Essentially \cref{lem:non-expansive-lemma} characterizes the explicit superiority of evaluating on-policy quantities over off-policy quantities. We believe this novel lemma is of independent interest for the field of OPE. The proof is postponed to the end of the section.
%
%\subsection{Outline of the Proof}
%In this section, we present the outline of the proof for \cref{th:dynkin_var}. We aim to use Markov chain CLT (\cite{jones2004markov}) to provide the asymptotic normality of our estimator. Note that Markov chain CLT states that for a Markov chain $X_{1}, X_{2}, \dotsc, $ and a bounded function $u$ with the domain on the state space, there exists $\Sigma_{u}$ such that
%\begin{align*}
%\sqrt{T}\left(\frac{1}{T}\sum_{t=1}^{T} u(X_t) - u^{*}\right) \overset{d}{\rightarrow} N(0, \Sigma_{u})
%\end{align*}
%where $u^{*}$ is the expected value of $u$ under the stationary distribution of the Markov chain. 
%
%\textbf{Delta method.} Unfortunately, the estimator $\tauDK$ can not be directly written as an empirical average of some function $u.$ To address this issue, we use ``delta method'' (traced back to \cite{doob1935limiting}, see \cref{lem:mapping-CLT}). In particular, we write $\tauDK = f(u_T)$ as a function of a random vector $u_{T}$ given by $u_{T} := \frac{1}{T}\sum_{t=1}^{T} u(X_{t}).$ Under some minor conditions, ``delta method'' states that 
%\begin{align*}
%\sqrt{T} \left(f(u_{T}) - f(u^{*})\right) \overset{d}{\rightarrow} N(0, \sigma_{f}^2)
%\end{align*}
%where $\sigma_{f}^2 := \nabla f(u^{*})^{\top} \Sigma_{u} \nabla f(u^{*})$ and $\nabla f(u^{*})$ is the gradient of $f$ evaluating at the point $u^{*}.$ This forms the basis of proving \cref{th:dynkin_var}. 
%
%\textbf{Linearization.} To simplify the analysis for $\sigma_{f}$, instead of computing $\Sigma_{u}$ explicitly, we ``linearize'' the function $f$ by defining $\tilde{f}(X_{t}) := \nabla f(u^{*})^{\top}(u(X_t)-u^{*})$ and the delta method in fact implies (see \cref{lem:linearization})
%\begin{align*}
%\sqrt{T}\left(\frac{1}{T}\sum_{t=1}^{T} \tilde{f}(X_t)\right) \overset{d}{\rightarrow} N(0, \sigma_{f}^2),
%\end{align*}
%i.e., the linearized $f$ converges with the same limiting variance as the original $f.$ Therefore, we can focus on $\tilde{f}$ for analyzing $\sigma_{f}.$ 
%
%\textbf{Bounding $\sigma_f$ with Entry-wise Non-expansive Lemma.} To bound $\sigma_{f}$, we will invoke \cref{lem:bound-for-sigma}, which states that
%\begin{align*}
%\sigma_{f} \leq \sqrt{2}\sqrt{\frac{2\ln(C)+1}{1-\lambda}}\tilde{f}_{\max}
%\end{align*}
%where $\tilde{f}_{\max} := \max_{s} |\tilde{f}(s)|.$ Then the problem boils down to bound $\tilde{f}_{\max}$, which will be controlled by \cref{lem:non-expansive-lemma}. 
%
%
%Next, we present the proof in full details. 
%\subsection{Delta Method and Linearization}
%To begin, consider the Markov chain $X_{t} = (s_{t}, a_{t}, s_{t+1}).$ For $a \in \{0, 1\}$, denote $F^{(a)}, h^{(a)}$ by
%\begin{align} \label{eq:def-F-h}
%F^{(a)}(X_t) &:= 2E_{s_t}E_{s_{t+1}}^{\top}\cdot 1(a_{t}=a)\\
%h^{(a)}(X_t) &:= 2r(s_t, a_t) \cdot E_{s_t}\cdot 1(a_t=a)
% \end{align}
% where $E_{s}$ is a vector with all entries zero except that the $s$-th entry is one. Let $F^{(a)}_{T} \in \R^{|\Sscr| \times |\Sscr|}, h^{(a)}_{T} \in \R^{|\Sscr|}$ be the empirical average of the function $F^{(a)}$ and $h^{(a)}$:
%\begin{align*}
%F^{(a)}_{T} &:= \frac{1}{T}\sum_{t=1}^{T} F^{(a)}(X_{t})\\
%h^{(a)}_{T} &= \frac{1}{T}\sum_{t=1}^{T} h^{(a)}(X_{t}).
%\end{align*} 
%We aim to write $\tauDK := f(F^{(0)}_T, F^{(1)}_T, h^{(0)}_T, h^{(1)}_T)$ as a function of $F^{(0)}_T, F^{(1)}_T, h^{(0)}_T, h^{(1)}_T$ for applying delta method. To do so, let $D_{T}^{(a)}$ be an diagonal matrix with entries $D_{T}^{(a)}(s, s) = \sum_{s'} F_{T}^{(a)}(s, s').$ One can verify that
%\begin{align*}
%\hat{V} = (D_{T}^{(0)}+D_{T}^{(1)} - F^{(0)}_T - F^{(1)}_F)^{\#} (h^{(0)}_T + h^{(1)}_{T})
%\end{align*}
%gives the estimation of $V$-function in \cref{eq:LSTD0-V}. Further, one can verify that with a plugging-in estimator for $Q$, the DQ estimator is given by 
%\begin{align*}
%\tauDK 
%&= f(F^{(0)}_T, F^{(1)}_T, h^{(0)}_T, h^{(1)}_T)\\
%&=: \one^{\top}(F^{(1)}_T-F^{(0)}_T)(D_{T}^{(0)}+D_{T}^{(1)} - F^{(0)}_T - F^{(1)}_F)^{\#} (h^{(0)}_T + h^{(1)}_{T})\\
%&\quad + \one^{\top} (h^{(1)}_T - h^{(0)}_T).
%\end{align*}
%By Markov chain CLT, we have when $T$ goes to infinity
%\begin{align*}
%F^{(0)}_T \rightarrow F^{*}_0 := DP_0,\quad  F^{(1)}_T \rightarrow F^{*}_1 := DP_1\\
%h^{(0)}_T \rightarrow h^{*}_0 := Dr_0,\quad  h^{(1)}_T \rightarrow h^{*}_1 := Dr_1
%\end{align*}
%where $D$ is a diagonal matrix with entries $D_{s,s} = \rho_{1/2}(s).$ Then by the delta method (see \cref{lem:mapping-CLT}), we have\footnote{The group inverse is continuous if we consider the set of matrices with rank $|\Sscr| - 1$ (\cite{rakovcevic1997continuity}).}
%\begin{align*}
%\sqrt{T} (f(F^{(0)}_T, F^{(1)}_T, h^{(0)}_T, h^{(1)}_T) - f(F^{*}_0, F^{*}_1, h^{*}_0, h^{*}_1)) \overset{d}{\rightarrow} N(0, \sigma_{f}^2)
%\end{align*}
%which is equivalent to 
%\begin{align*}
%\sqrt{T} (\tauDK - \E_{\rho_{1/2}}[\tauDK]) \overset{d}{\rightarrow} N(0, \sigma_{f}^2)
%\end{align*}
%since $ f(F^{*}_0, F^{*}_1, h^{*}_0, h^{*}_1) = \E_{\rho_{1/2}}[\tauDK].$ To analyze $\sigma_{f}$, we consider the ``linearization'' of $f$ around $u^{*} := (F^{*}_0, F^{*}_1, h^{*}_0, h^{*}_1).$ In particular, let $u(X_t) = (F^{(0)}(X_t), F^{(1)}(X_t), h^{(0)}(X_t), h^{(1)}(X_t)).$ Let $(\lambda, V)$ be the average reward and the ``true'' $V$-function under the policy $\pi_{1/2}.$ One can verify that
%\begin{align*}
% \tilde{f}(s,a,s')&:=\nabla f(u^{*})^{\top}(u(s, a, s')-u^{*}) \\
% &= (\one^{\top}D(P_1-P_0)(I-P_{1/2})^{\#}D^{-1})E_{s} (r(s,a)-\lambda + V(s') - V(s)) \\
% &\quad + 2(1(a=1)-1(a=0))(V(s') + r(s, a)) - c
%\end{align*}
%where $c := \E_{\rho_{1/2}}[2(1(a=1)-1(a=0))(V(s') + r(s, a)-\lambda)].$ By \cref{lem:linearization}, we have
%\begin{align*}
%\sqrt{T}\left(\frac{1}{T}\sum_{t=1}^{T} \tilde{f}(X_t)\right) \overset{d}{\rightarrow} N(0, \sigma_{f}^2).
%\end{align*}
%Here $\sigma_{f}^2$ is explicitly given by (by Markov Chain CLT)
%\begin{align*}
%\sigma_{f}^2 
%&:= \sum_{s,a,s'} \tilde{f}(s,a,s')^2 \rho_{1/2}(s)P_{a}(s, s') \frac{1}{2} \\
%&\quad + 2\sum_{s,a,s'} \rho_{1/2}(s)P_{a}(s,s')\frac{1}{2}\tilde{f}(s,a,s') \sum_{s_1} (I-P_{1/2})^{\#}_{s',s_1} t(s_1)
%\end{align*}
%where $t(s) = \sum_{a,s'} \tilde{f}(s,a,s')P_{a}(s,s')\rho_{1/2}(s)\frac{1}{2}.$
%
%%let $P^{(0)}_{T}, P^{(1)}_{T}$ be the empirical transition matrix of $\pi_0$ and $\pi_1$ derived from $F^{(0)}_T, F^{(1)}_T$, i.e., 
%%\begin{align*}
%%P^{(0)}_{T}(s, s') = \frac{F^{(0)}_T(s, s')}{\sum_{s''} F^{(0)}_T(s, s'')}, \quad P^{(1)}_{T}(s, s') = \frac{F^{(1)}_T(s, s')}{\sum_{s''} F^{(1)}_T(s, s'')}.
%%\end{align*}
%
%
%
%%note that
%%\begin{align*}
%%(F^{(0)} + F^{(1)})\hat{V}
%%\end{align*}
%
%\subsection{Bound $\sigma_{f}$}
%Next, we aim to provide a bound for $\sigma_{f}.$ Note that that the mixing time of $X_{t}$ is the same as $s_{t}$ and by \cref{lem:bound-for-sigma}, we have
%\begin{align*}
%\sigma_{f} \leq \sqrt{2}\tilde{f}_{\max} \sqrt{\frac{2\ln(C)+1}{1-\lambda}}
%\end{align*}
%where $\tilde{f}_{\max} = \max_{s,a,s'} |\tilde{f}(s,a,s')|.$ Then the problem boils down to bound $\tilde{f}_{\max}.$ 
%
%Let $z_{s} := (\one^{\top}D(P_1-P_0)(I-P_{1/2})^{\#}D^{-1})E_{s}.$ By the definition of $\tilde{f}$, we have
%\begin{align*}
%\tilde{f}_{\max} \leq 2(z_{\max}+2) (V_{\max} + r_{\max})
%\end{align*}
%where $z_{\max} := \max_{s} |z_{s}|, V_{\max} := \max_{s} |V(s)|.$ For $V_{\max}$, we have
%\begin{align*}
%\norm{V}_{\infty} 
%&= \norm{(I-P_{1/2})^{\#} r}_{\infty}\\
%&\leq \norm{(I-P_{1/2})}_{1,\infty} r_{\max}\\
%&\leq \frac{2\ln(C)+1}{1-\lambda} r_{\max}.
%\end{align*}
%For $z_{\max}$, note that
%\begin{align*}
%z_{s} 
%&= \one^{\top}D(P_1-P_0)(I-P_{1/2})^{\#}D^{-1})E_{s}\\
%&= \rho_{1/2}^{\top} (P_1-P_0)(I-P_{1/2})^{\#} D^{-1} E_s\\
%&= \rho_{1/2}^{\top} (P_1-P_0)(I-P_{1/2})^{\#}E_s \frac{1}{\rho_{1/2}(s)}.
%\end{align*}
%Then, we can invoke \cref{lem:non-expansive-lemma} to obtain that 
%\begin{align*}
%z_{s} = W(\rho_{1/2})(s) \frac{1}{\rho_{1/2}(s)} \leq 4\frac{\ln(C) +  \ln \left(1/\rho_{\min}\right) + 1}{1-\lambda}.
%\end{align*}
%Combining all together, we have
%\begin{align*}
%\sigma_{f} \leq C' \log\left(\frac{1}{\rho_{\min}}\right) \left(\frac{1}{1-\lambda}\right)^{5/2} r_{\max}
%\end{align*}
%for some constant $C'$ that depends (polynomially) on $\log(C)$, which completes the proof of \cref{th:dynkin_var}.
%
%\subsection{Proof of \cref{lem:non-expansive-lemma}}
%The only thing remaining is the proof of \cref{lem:non-expansive-lemma}. 
%
%Note that we have $W(\rho^{1/2}) = (I-P_{1/2})^{\#\top}(P_1-P_0)^{\top} \rho_{1/2}.$ Let $v:= (P_1 - P_0)^{\top} \rho_{1/2}$. We will show first (i) $\frac{1}{2} v$ is entry-wise non-expansive; and then (ii) $(I-P_{1/2})^{\top}v$ is entry-wise bounded. 
% 
%To begin, we claim that $|(P_1-P_0)(s,s')| \leq 2 P_{1/2}(s,s')$ for any $s$ and $s'.$ This is due to $2P_{1/2} = P_{0} + P_{1}$ and for any $a\geq 0, b\geq 0$, we have $|a-b| \leq a+b$.
%
%Furthermore, note that $\rho_{1/2}^{\top} P_{1/2} = \rho_{1/2}^{\top}.$ Then for any $s'$, 
%\begin{align*}
%|v(s')| 
%&= \left|\sum_{s} \rho_{1/2}(s) (P_{1}-P_{0})_{s, s'}\right|\\
%&\leq \sum_{s} \rho_{1/2}(s) | (P_{1}-P_{0})_{s, s'}|\\
%&\leq \sum_{s} \rho_{1/2}(s) 2 P_{1/2}(s,s')\\
%&\leq 2 \rho_{1/2}(s').
%\end{align*}
%This is to say, $\frac{v}{2}$ is entry-wise bounded by $\rho_{1/2}$. Furthermore, this bound continues to hold after any transformation for $v$ under $P_{1/2}$:
%\begin{align*}
%|(v^{\top}P_{1/2}^{k})(s')| 
%&= \left|\sum_{s} v(s) P_{1/2}^{k}(s, s')\right|\\
%&\leq 2\sum_{s} \rho_{1/2}(s) P_{1/2}^{k}(s, s')\\
%&\leq 2\rho_{1/2}(s').
%\end{align*}
%
%Next, consider
%\begin{align*}
%v^{\top}(I-P_{1/2})^{\#}E_{s}
%&= \sum_{k=0}^{\infty} v^{\top} (P_{1/2}^{k} - \one\rho_{1/2}^{\top})E_{s}\\
%&=: \sum_{k=0}^{\infty} a_{k}.
%\end{align*}
%Note that $|(v^{\top}P_{1/2}^{k})E_{s}| \leq 2 \rho_{1/2}(s).$ Further, $|v^{\top}\one\rho_{1/2}^{\top}E_{s}| \leq |v^{\top} \one| \rho_{1/2}(s) \leq 2\rho_{1/2}(s).$ Therefore, for any $k$,  $|a_{k}| \leq 4\rho_{1/2}(s).$
%We also have
%\begin{align*}
%|a_{k}| 
%&\leq \norm{v^{\top}}_{1} \norm{P^{k}-\one\rho^{\top}}_{1,\infty} \norm{E_{s}}_{\max}\\
%&\leq 2 C\lambda^{k}.
%\end{align*}
%Using the same trick in proving \cref{lem:group-inverse-L1}, we have
%\begin{align*}
%\frac{1}{\rho_{1/2}(s)}\sum_{k=0}^{\infty} |a_{k}| 
%&\leq\sum_{k=0}^{\infty} \min\left(4, 2 C\lambda^{k} \frac{1}{\rho_{1/2}(s)}\right) \\
%&\leq 2\left(\sum_{k=0}^{\log_{\lambda}(C/\rho_{1/2}(s))-1} 2 + \sum_{k=\log_{\lambda}(C/\rho_{1/2}(s))} \frac{C}{\rho_{1/2}(s)} \lambda^{k}\right)\\
%&= \frac{4\ln(C/\rho_{1/2}(s))}{-\ln(\lambda)} + \frac{2}{1-\lambda}\\
%&\leq \frac{4\ln(C/\rho_{1/2}(s))}{1-\lambda} + \frac{2}{1-\lambda}\\
%&\leq 4\frac{\ln(C) +  \ln \left(1/\rho_{\min}\right) + 1}{1-\lambda}.
%\end{align*}
%Then $\left|W(\rho_{1/2})(s)\right| = |\sum_{k}a_{k}| \leq c \rho_{1/2}(s)$ with $c := 4\frac{\ln(C) +  \ln \left(1/\rho_{\min}\right) + 1}{1-\lambda}.$ This completes the proof.
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> Tex Files/Variance.tex <==
\section{The Price of Being Unbiased} \label{sec:price}
Thus far, we have seen that the DQ estimator provides a dramatic mitigation in bias (Theorem~\ref{th:dynkin_bias}) at a relatively modest price in variance (Theorem~\ref{th:dynkin_var}). This suggests another question: could we hope to construct an {\em unbiased} estimator that has low variance (i.e. comparable to either the Naive or DQ estimators). We will see that the short answer is: no. 


\subsection{The Variance of an Optimal Unbiased Estimator}

As noted earlier, a plethora of Off-policy evaluation (OPE) algorithms might be used to provide an unbiased estimate of the ATE. Rather than consider a particular OPE algorithm, here we produce a Cram\'{e}r-rao lower bound on the variance of {\em any} unbiased OPE algorithm. While such a bound is obviously of independent interest (since OPE is a far more general problem than what we seek to accomplish in this paper), we will primarily be interested in comparing this lower bound to the variance of the DQ estimator from Theorem~\ref{th:dynkin_var}.

\begin{theorem}[Variance Lower Bound for Unbiased Estimators]
\label{th:cramer-rao}
Assume we are given a dataset  $\{(s_t,a_t, r(s_t,a_t)): t=0, \dots,T \}$ generated under the experimentation policy $\pi_{1/2}$, with $s_0$ distributed according to $\rho_{1/2}$.  Then for any unbiased estimator $\hat{\tau}$ of $\mathrm{ATE}$, we have that
\begin{align*}
T\cdot \mathrm{Var}(\hat{\tau}) 
&\geq 2\sum_{s} \frac{\rho_1(s)^2}{\rho_{1/2}(s)} \sum_{s'} p(s, 1, s')(V_{\pi_1}(s') - V_{\pi_1}(s) + r(s,1) - \lambda^{\pi_1})^2\\
&\quad + 2\sum_{s} \frac{\rho_0(s)^2}{\rho_{1/2}(s)} \sum_{s'} p(s, 0, s')(V_{\pi_0}(s') - V_{\pi_0}(s) + r(s,0) - \lambda^{\pi_0})^2 \triangleq \sigoff^2.
\end{align*}
\end{theorem}

It is worth remarking that this lower bound is tight: in the appendix we show that an LSTD(0)-type OPE algorithm achieves this lower bound. While this is of independent interest vis-\`{a}-vis 
average cost OPE, we turn next to our ostensible goal here -- evaluating the `price' of unbiasedness. We can do so simply by comparing the variance of the DQ estimator with the lower bound above. In fact, we are able to exhibit a class of one-dimensional Markov chains (in essence the model in \cref{sec:example}) for which we have: 

\begin{theorem}[Price of Unbiasedness]
\label{th:price}
    For any $0 < \delta \leq \frac{1}{5}$, there exists a class of MDPs parameterized by $n \in\mathbb{N}$, where $n$ is the number of states, such that   $\frac{\sigma_{\rm DQ}}{\sigoff} = O\left(\frac{n}{c^{n}}\right),$
    for some constant $c>1$. Furthermore, $|(\mathrm{ATE}-\E[\hat{\mathrm{ATE}}_{\rm DQ}])/\mathrm{ATE}| \leq \delta.$
\end{theorem}

\noindent\textbf{\textsf{Another Extreme of the Bias-Variance Tradeoff:}} Theorems~\ref{th:dynkin_var}, \ref{th:cramer-rao}, and \ref{th:price} together reveal the opposite extreme of the bias-variance tradeoff. Specifically, if we insisted on an unbiased estimator for our problem (of which there are many, thanks to our framing of the problem as one of OPE), we would pay a large price in terms of variance. In particular Theorem~\ref{th:price} illustrates that this price can grow exponentially in the size of the state space. This jibes with our empirical evaluation in both caricatured and large-scale MDPs in Section~\ref{sec:experiments}. 

Taken together our results reveal that the DQ estimator accomplishes a striking bias-variance tradeoff: it has substantially smaller variance than any unbiased estimator (in fact, comparable to the Naive estimator), all while ensuring bias that is second order in the impact of the intervention.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

